Correlated Quantal Response Equilibrium: A New Equilibrium Notion for Human-AI Strategic Interactions

The modeling of the behavior of agents in strategic environments and the prediction of the resulting outcomes has long been a challenging problem; this has been the focus of game theory. The introduction of AI agents as human-aids or as sole decision-makers expands the underlying question: Can we model behavior and predict outcomes of strategic games that involve a mix of AI agents and human players? As an initial answer, we propose Correlated Quantal Response Equilibrium (CQRE) that combines and generalizes classical solution concepts such as Quantal Response Equilibrium and Correlated Equilibrium. We answer questions of existence and propose a method for computing the CQRE that is a best fit to a given joint action distribution. We demonstrate the empirical effectiveness of CQRE predictions using a diverse collection of complex general-sum games, including high-rank and large-action two-player games, challenging multiplayer games, and a large-scale extension of the Selten--Chmura setting to AI--AI and human--AI play.

==> intro-v1.tex <==
\section{Introduction}
Large language models are increasingly deployed as decision-making agents alongside humans and other AI systems. In such settings, behavior is described not only by each player's marginal action frequencies but by the joint distribution over all players' actions: which outcomes occur together and how choices vary across roles and populations. This joint perspective is essential for comparing human--human, human--AI, and AI--AI behavior and for more general multiplayer interactions. However, these scenarios are typically studied in isolation, and a common framework to model joint strategic behavior in them is limited.

Classical mixed Nash equilibrium~\citep{nash1951noncoop} imposes exact best responses and independent randomization between players. Logit-QRE~\citep{mckelvey1995qre,goeree2005regular} softens best response through payoff-sensitive stochastic choice and is widely used to describe experimental human play~\citep{selten2008stationary}, but it retains independent randomization between players. Correlated equilibrium~\citep{aumann1974subjectivity,aumann1987correlated} allows for coordination and cross-player dependence by studying joint distributions. However, it requires exact obedience to every recommendation and yields a set of distributions rather than a unique prediction. What is missing is a point prediction over joint actions that represents dependence while permitting heterogeneous action-specific deviations from exact obedience.


To fill this gap, we introduce \emph{correlated quantal response equilibrium with per-action slack} (CQRE-pa) for general finite $N$-player games. For each player $i$ and recommended action $a_i$, a nonnegative slack $\gamma_{i,a_i}$ bounds the recommendation-weighted payoff gain from any unilateral deviation. Among all joint distributions satisfying these relaxed obedience constraints, CQRE-pa selects the one with maximum Shannon entropy, equivalently the feasible distribution closest to uniform~\citep{jaynes1957information}. This rule yields a unique prediction for every fixed slack vector. We also consider two specializations that isolate the value of action-specific flexibility: scalar CQRE shares one slack across all players and actions, whereas per-player CQRE assigns one slack to each player; CQRE-pa assigns a separate slack to every player--action pair.

Fixing the per-action slacks defines an inner optimization problem that selects the unique maximum-entropy joint distribution that satisfies the relaxed obedience constraints. Because the appropriate slacks for observed play in a given game are not known in advance, we introduce an outer optimization problem that searches over slack vectors and minimizes the KL divergence between the inner solution and the empirical joint-action distribution. Together, these two problems form a bi-level estimator of CQRE-pa. 

We evaluate CQRE-pa across human and LLM play in two- and three-player games. Relative to fitted Logit-QRE, CQRE-pa reduces mean KL by 56.9\% on the twelve actual human plays' games, achieves lower aggregate KL on AI--AI targets, has lower mean KL in six of seven larger-action games, and is favored in all 56 three-player comparisons. Logit-QRE remains better on constructed product-form human--AI target games. To support this evaluation, we contribute 201,600 accepted one-shot decisions from six OpenAI model deployments across all twelve Selten--Chmura games. Combined with published human data, these observations support 588 targets: 432 AI--AI, 144 constructed directional human--AI, and 12 human--human.

\paragraph{Contributions.} Our contributions are threefold:
    \begin{enumerate}
      \item We introduce CQRE-pa (and specializations) for general finite-player games, prove existence and uniqueness for any slack vector, establish nesting of scalar, per-player, and per-action versions, and derive an exponential-family characterization.
      \item Given a (empirically obtained) joint action distribution, we formulate the problem of finding the closest CQRE-pa (and the specializations) as a bi-level optimization problem and provide an implementation---at the lower level finding the CQRE-pa given a choice of slack variables, and at the higher level optimizing the slack variables to obtain the best fit (to the given joint action distribution). The nested CQRE specializations provide ablations of action-specific flexibility.
      \item We also contribute a reproducible LLM decision dataset and evaluate CQRE-pa across established human behavior, human and AI populations, larger action spaces, different payoff structures, and three-player play, which for most cases CQRE-pa is a better notion.     
  \end{enumerate}

\paragraph{Related work.}
  CQRE-pa connects three lines of research. QRE and its generalizations model bounded rationality through stochastic or regularized player-level responses~\citep{mckelvey1995qre,goeree2005regular,zhao2026efficient}, but their joint predictions remain products of individual mixed strategies. Correlated equilibrium incorporates coordination, where the maximum-entropy correlated equilibrium provides a unique selection from the set of correlated-equilibria~\citep{aumann1974subjectivity,aumann1987correlated,ortiz2007maximum}. CQRE-pa combines maximum-entropy selection with action-indexed relaxations of obedience and estimates
  those relaxations from observed joint play. Recent work also studies LLMs as strategic players and documents sensitivity to game structure and presentation~\citep{akata2023playing,lore2024strategicllms,fan2024gametheory,pezeshkpour2024llmsensitivity,zheng2024llmrobustchoice}; our focus is a common equilibrium framework for comparing complete joint distributions across human and AI populations.

Section~\ref{sec:cqre} defines CQRE-pa and establishes its theoretical properties. Section~\ref{sec:compute} presents the bilevel estimation procedure. Section~\ref{sec:dataset} describes the datasets and experimental design, and Section~\ref{sec:empirical} reports the empirical evaluation. The appendix contains complete proofs, computational and experimental details, additional results, and reproducibility information.

% \begin{itemize}
% \item Motivation: AI systems increasingly interact strategically with humans and other AI systems. Understanding them requires studying joint outcomes, not only isolated decisions. comparisons of human–human, human–AI, and AI–AI joint behavior under a common framework remain limited.
% \end{itemize}

% Classical (mixed) Nash equilibrium~\citep{nash1951noncoop} is too rigid for noisy agents. Quantal response
% equilibrium~\citep{mckelvey1995qre,goeree2005regular} relaxes best response via a softmax with a single inverse-temperature per player, and is the standard relaxation for human experimental data~\citep{selten2008stationary}. Correlated equilibrium~\citep{aumann1974subjectivity,aumann1987correlated} permits joint recommendations but no per-action mistakes.

% \begin{itemize}
% \item Recent research...

% \item Our methods: We introduce CQRE-pa, which relaxes correlated-equilibrium obedience constraints using per-action slacks. For fixed slacks, CQRE-pa selects a unique maximum-entropy joint distribution; the slacks are then estimated through continuous optimization against observed play.

% \item CQRE-pa addresses two structural restrictions of Logit-QRE: product-form joint play and the use of one precision parameter per player. CQRE-pa models joint distributions directly and assigns one slack to each (player, action) pair, allowing it to accommodate non-product dependence and action-specific asymmetries.
% \end{itemize}

% We define CQRE-pa as the maximum-entropy correlated strategy in a closed convex polytope parameterized by a nonnegative slack vector $\gamma\in\Real_+^{\sum_{i\in\mathcal N}|A_i|}$, and prove existence, uniqueness, and an exponential-family closed form in Section~\ref{sec:cqre}. Section~\ref{sec:compute} specifies the convex solver, the discrete slack grid and the continuous bilevel outer-slack estimator, the five comparison notions (mixed Nash, Logit-QRE, exact CQRE, scalar CQRE, per-player CQRE), and the paired bootstrap test. Section~\ref{sec:empirical} reports the empirical evaluation on three independent datasets.

% \begin{itemize}
%     \item Our Contributions...
%     \item Related Works...
% \end{itemize}



==> old_info/paper/algorithm.tex <==
\section{Computing a CQRE}
\label{sec:compute-cqre}

Having defined CQRE as the unique optimizer of a maximum-entropy program, we now describe how it is computed in the finite-game setting. The key point is that CQRE is a convex optimization problem with an entropy objective and linear obedience constraints, so generic constrained optimization routines can be used directly.

For the $2\times2$ games used in our numerical experiments, the optimization variable is the four-cell joint distribution
\begin{equation}
\rho = \bigl(\rho(U,L),\rho(U,R),\rho(D,L),\rho(D,R)\bigr).
\end{equation}
The feasible region is the probability simplex together with four linear deviation constraints,
\begin{align}
\sum_{a_2}\rho(U,a_2)\bigl(U_1(D,a_2)-U_1(U,a_2)\bigr) &\le \gamma_U,
\label{eq:compute-u-to-d}\\
\sum_{a_2}\rho(D,a_2)\bigl(U_1(U,a_2)-U_1(D,a_2)\bigr) &\le \gamma_D,
\label{eq:compute-d-to-u}\\
\sum_{a_1}\rho(a_1,L)\bigl(U_2(a_1,R)-U_2(a_1,L)\bigr) &\le \gamma_L,
\label{eq:compute-l-to-r}\\
\sum_{a_1}\rho(a_1,R)\bigl(U_2(a_1,L)-U_2(a_1,R)\bigr) &\le \gamma_R.
\label{eq:compute-r-to-l}
\end{align}
The objective is
\begin{equation}
F(\rho)=\sum_{a_1,a_2}\rho(a_1,a_2)\log\rho(a_1,a_2).
\end{equation}
Since the feasible set is compact and convex and the objective is strictly convex, the optimization problem has a unique solution by Theorems~\ref{thm:cqre-existence} and~\ref{thm:cqre-uniqueness}.

\paragraph{Payoff normalization.}
When comparing relaxation levels across different games, the numerical value of $\gamma$ depends on the utility scale. In the Selten--Chmura benchmark we therefore normalize payoffs game by game. For player $i\in\{1,2\}$ and game $g$, define the maximum unilateral deviation scale
\begin{equation}
\Delta_i(g)=\max_{a_i,\widetilde a_i,a_{-i}}\bigl|\bar U_i^{(g)}(\widetilde a_i,a_{-i})-\bar U_i^{(g)}(a_i,a_{-i})\bigr|,
\qquad
U_i^{(g)}=\bar U_i^{(g)}/\Delta_i(g).
\label{eq:payoff-normalization}
\end{equation}
This preserves the direction of every unilateral deviation while putting the relaxation parameters on a common scale.

\paragraph{Grid search over relaxation families.}
For scalar, per-player, and per-action CQRE, we evaluate CQRE over a finite candidate set of relaxation values and choose the value or vector that best fits the target empirical distribution for the benchmark under study. In the direct Selten--Chmura fitting experiment, the grid is
\begin{equation}
\Gamma_0=\{0,0.005,0.01,0.02,0.05,0.1,0.2\}.
\end{equation}
For the scalar family this is a one-dimensional search over $\epsilon$; for the per-player family it induces a two-dimensional search over $(\epsilon_1,\epsilon_2)$; and for the per-action family it induces a four-dimensional search over $(\gamma_U,\gamma_D,\gamma_L,\gamma_R)$.

\paragraph{Relation to other benchmarks.}
The same computational framework also covers the exact CQRE / maximum-entropy correlated-equilibrium benchmark by setting $\gamma=0$. In the Selten--Chmura constant-sum games this exact benchmark coincides numerically with the mixed Nash product. For comparison with independent benchmarks such as Nash and logit QRE, we always map the predicted strategies to a joint distribution before measuring the fit to data.


==> old_info/paper/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> old_info/paper/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We introduced CQRE as a maximum-entropy relaxation of correlated equilibrium and showed that it is well defined for finite games.  Empirically, exact CE/Nash is too rigid on both human and LLM-generated data, while relaxed CQRE gives substantially better joint-distribution fits.  Product-form logit QRE remains the key benchmark: it is strongest on the Selten--Chmura human data, while per-action CQRE is competitive under bootstrap uncertainty and is strongest or statistically tied in several LLM one-shot benchmarks.  The broad conclusion is that relaxed obedience provides a useful way to model empirical deviations from exact equilibrium, especially when action-specific or model-specific biases create joint behavior that is not well captured by exact CE/Nash.


==> old_info/paper/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The experiments give a mixed but informative picture.  Exact CQRE, which is the maximum-entropy CE benchmark, coincides with the mixed Nash product in the Selten--Chmura constant-sum games and in the weighted-RPS LLM experiments.  In all empirical settings this exact benchmark fits poorly, suggesting that exact obedience is too restrictive for empirical joint play.

Relaxation changes the picture substantially.  On the human data, all relaxed CQRE variants improve over exact CQRE/Nash by nearly an order of magnitude in mean KL.  The per-action variant is the best CQRE parameterization, but the per-game logit-QRE product has the best point estimate.  Bootstrap intervals show that the gap between logit QRE and per-action CQRE is not cleanly separated, so the correct interpretation is that relaxed CQRE is competitive with a strong product-form benchmark rather than uniformly dominant on the human dataset.

The LLM experiments show a complementary pattern.  In the local Qwen shared-signal pilot, per-action CQRE has the smallest point-estimate KL, while logit QRE is extremely close and its bootstrap interval overlaps with CQRE.  The larger GPT round-robin gives a sharper view: per-action CQRE weakly dominates Nash, exact CQRE, and the nested CQRE scalar/per-player families on every completed pair, and it often improves on logit QRE in the high-deviation regimes where product-form QRE struggles.  At the same time, many cross-model pairs lie close to the QRE--CQRE diagonal, so the evidence should be read as support for CQRE as a competitive and flexible joint-distribution benchmark, not as a proof that QRE is obsolete.

A limitation of the current empirical analysis is that QRE and CQRE parameters are fit to each benchmark rather than predicted from game features.  This is intentional for the current paper: our goal is to test whether relaxed obedience can describe empirical joint play at all.  A stronger future benchmark would fit a small number of relaxation parameters across many games, or derive the relaxation vector from payoff features, model uncertainty, or prompt-level information.  Another limitation is sample size for the LLM experiments: although the round-robin provides broad model coverage, each pair currently uses $N=200$ one-shot matches.  Larger samples would tighten bootstrap intervals and clarify whether the small QRE--CQRE gaps in low-KL regimes are meaningful.


==> old_info/paper/formulation.tex <==
\section{Correlated Quantal Response Equilibrium}
\label{sec:cqre}

We consider a finite two-player normal-form game with action sets $A_1$ and $A_2$ and utility functions $U_1$ and $U_2$. A joint distribution $\rho\in\Delta(A_1\times A_2)$ specifies how often each action pair $(a_1,a_2)$ is played. For player $1$, fixing a recommended action $a_1$, define the reweighted utility
\begin{equation}
\widetilde U_{1,a_1}(\widetilde a_1,a_2)=\rho(a_1,a_2)U_1(\widetilde a_1,a_2).
\end{equation}
Then the correlated-equilibrium obedience condition can be written as
\begin{equation}
\delta_{a_1}
\in
\arg\max_{\pi_1\in\Delta(A_1)}
\sum_{\widetilde a_1,a_2}
\pi_1(\widetilde a_1)\widetilde U_{1,a_1}(\widetilde a_1,a_2),
\qquad \forall a_1\in A_1,
\label{eq:obedience-player1}
\end{equation}
with an analogous condition for player $2$. Writing obedience in this reweighted form avoids the usual conditioning issue when $\rho(a_i)=0$.

\begin{definition}[CQRE feasible set]
For a nonnegative relaxation vector $\gamma=(\gamma_{a_1})_{a_1\in A_1}\cup(\gamma_{a_2})_{a_2\in A_2}$, define $K_\gamma\subseteq\Delta(A_1\times A_2)$ as the set of joint distributions satisfying
\begin{align}
\sum_{a_2\in A_2}\rho(a_1,a_2)U_1(a_1,a_2)
&\ge
\max_{\pi_1\in\Delta(A_1)}
\sum_{\widetilde a_1,a_2}
\pi_1(\widetilde a_1)\rho(a_1,a_2)U_1(\widetilde a_1,a_2)-\gamma_{a_1},
\quad \forall a_1\in A_1,
\label{eq:cqre-feasible-p1}\\
\sum_{a_1\in A_1}\rho(a_1,a_2)U_2(a_1,a_2)
&\ge
\max_{\pi_2\in\Delta(A_2)}
\sum_{a_1,\widetilde a_2}
\pi_2(\widetilde a_2)\rho(a_1,a_2)U_2(a_1,\widetilde a_2)-\gamma_{a_2},
\quad \forall a_2\in A_2.
\label{eq:cqre-feasible-p2}
\end{align}
\end{definition}

\begin{definition}[Correlated quantal response equilibrium]
For a fixed relaxation vector $\gamma\ge 0$, a \emph{correlated quantal response equilibrium} is the unique maximum-entropy point in $K_\gamma$:
\begin{equation}
\rho_\gamma^{\star}
\in
\arg\min_{\rho\in K_\gamma}
\sum_{(a_1,a_2)\in A_1\times A_2}\rho(a_1,a_2)\log \rho(a_1,a_2).
\label{eq:cqre-optimization}
\end{equation}
When $\gamma=0$, the feasible set is exactly the set of correlated equilibria, so \eqref{eq:cqre-optimization} selects the maximum-entropy correlated equilibrium.
\end{definition}

The obedience constraints admit an equivalent linear deviation form. For player $1$, \eqref{eq:cqre-feasible-p1} is equivalent to
\begin{equation}
\sum_{a_2\in A_2}\rho(a_1,a_2)\bigl(U_1(\widetilde a_1,a_2)-U_1(a_1,a_2)\bigr)
\le \gamma_{a_1},
\qquad \forall a_1\in A_1,\ \forall \widetilde a_1\in A_1\setminus\{a_1\},
\label{eq:linear-dev-p1}
\end{equation}
and analogously for player $2$.

\begin{proposition}[Exponential-family form]
Let $\lambda_{a_i,\widetilde a_i}\ge 0$ denote the Lagrange multiplier associated with the deviation constraint from $a_i$ to $\widetilde a_i$. Then any optimizer of \eqref{eq:cqre-optimization} satisfies
\begin{equation}
\rho(a_1,a_2)
\propto
\exp\Bigg(
\sum_{\widetilde a_1\in A_1\setminus\{a_1\}}
\lambda_{a_1,\widetilde a_1}\bigl(U_1(a_1,a_2)-U_1(\widetilde a_1,a_2)\bigr)
+
\sum_{\widetilde a_2\in A_2\setminus\{a_2\}}
\lambda_{a_2,\widetilde a_2}\bigl(U_2(a_1,a_2)-U_2(a_1,\widetilde a_2)\bigr)
\Bigg).
\label{eq:exp-family-cqre}
\end{equation}
\end{proposition}

\begin{proof}
The objective in \eqref{eq:cqre-optimization} is the negative Shannon entropy up to sign. Introducing multipliers for the simplex constraint and the linear deviation constraints and differentiating the Lagrangian with respect to $\rho(a_1,a_2)$ yields the stated Gibbs form after exponentiation and normalization.
\end{proof}

\begin{theorem}[Existence]
\label{thm:cqre-existence}
Let $A_1$ and $A_2$ be finite, let $U_1,U_2$ be bounded, and let $\gamma\ge 0$. Then the optimization problem \eqref{eq:cqre-optimization} admits at least one minimizer.
\end{theorem}

\begin{proof}
Let $K_\gamma$ denote the feasible set. Because the game is finite, there exists a mixed Nash equilibrium $(\sigma_1,\sigma_2)$. The associated product distribution $\bar\rho(a_1,a_2)=\sigma_1(a_1)\sigma_2(a_2)$ satisfies all obedience constraints with slack at most $0$, hence $\bar\rho\in K_\gamma$ whenever $\gamma\ge 0$. Therefore $K_\gamma$ is nonempty. Since the deviation constraints are linear in $\rho$, $K_\gamma$ is a closed subset of the simplex $\Delta(A_1\times A_2)$, which is compact in finite dimensions. Finally, with the convention $0\log 0:=0$, the objective is continuous on $K_\gamma$. By the Weierstrass theorem, a minimizer exists.
\end{proof}

\begin{theorem}[Uniqueness]
\label{thm:cqre-uniqueness}
Under the assumptions of Theorem~\ref{thm:cqre-existence}, the optimization problem \eqref{eq:cqre-optimization} admits a unique minimizer.
\end{theorem}

\begin{proof}
The feasible set $K_\gamma$ is convex because it is the intersection of the simplex with linear constraints. The function $x\mapsto x\log x$ is strictly convex on $[0,1]$, so
\begin{equation}
F(\rho)=\sum_{(a_1,a_2)\in A_1\times A_2}\rho(a_1,a_2)\log \rho(a_1,a_2)
\end{equation}
is strictly convex on $\Delta(A_1\times A_2)$ and hence on $K_\gamma$. A strictly convex function has at most one minimizer on a convex feasible set, so the minimizer is unique.
\end{proof}

In the $2\times 2$ experiments below we will consider three nested relaxation families. Writing $A_1=\{U,D\}$ and $A_2=\{L,R\}$, we study
\begin{align}
\text{scalar: } &\gamma_U=\gamma_D=\gamma_L=\gamma_R=\epsilon, \\
\text{per-player: } &\gamma_U=\gamma_D=\epsilon_1,\qquad \gamma_L=\gamma_R=\epsilon_2, \\
\text{per-action: } &\gamma=(\gamma_U,\gamma_D,\gamma_L,\gamma_R).
\end{align}
These families are not part of the definition of CQRE itself; they are empirical parameterizations used to study how much relaxation the human and synthetic data seem to require.


==> old_info/paper/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Equilibrium concepts are often used as compact descriptions of strategic behavior, but exact equilibrium predictions can be too rigid when agents are noisy, boundedly rational, or only approximately obedient to recommendations.  Quantal response equilibrium (QRE) relaxes exact best-response behavior by allowing payoff-sensitive mistakes, while correlated equilibrium (CE) allows joint recommendations and correlation across players.  This paper studies a simple bridge between these ideas: a correlated equilibrium-style joint distribution selected by maximum entropy under relaxed obedience constraints.

Our goal is not to model the full dynamics by which agents learn to play a game.  Instead, we ask whether a static joint distribution derived from the payoff matrix can explain empirical joint play.  This is natural for population-style random-matching experiments and for one-shot LLM self-play data, where the observable object is an empirical distribution over action pairs.  We therefore evaluate each candidate equilibrium notion by comparing its predicted joint distribution to the empirical joint distribution using KL divergence.

We make three contributions.  First, we define correlated quantal response equilibrium (CQRE) as the unique maximum-entropy solution of a convex program over relaxed obedience constraints, and prove existence and uniqueness for finite two-player games.  Second, we describe how CQRE is computed in finite games and study scalar, per-player, and per-action relaxations.  Third, we evaluate CQRE on human and LLM benchmarks: the Selten--Chmura constant-sum human data, a local Qwen weighted rock--paper--scissors pilot, and a larger round-robin of GPT model pairs on the same weighted game.  In all settings exact CE/Nash is too rigid, while relaxed CQRE gives a substantially better fit.  On the human data, logit QRE has the lowest mean KL, but per-action CQRE is close with overlapping bootstrap confidence intervals.  On the LLM data, per-action CQRE is competitive with logit QRE and is especially useful in high-deviation self-play and intra-family model-pair regimes.  These results support CQRE as a useful relaxed joint-distribution benchmark rather than as a uniformly dominant replacement for QRE.


==> old_info/paper/numerical-experiments.tex <==
\section{Numerical Results}
\label{sec:numerical}

We evaluate CQRE as a predictor of empirical \emph{joint} play.  In all experiments the target is an empirical distribution over action pairs and each equilibrium notion is mapped to a joint distribution before evaluation.  If $\widehat\rho$ denotes an empirical joint distribution and $Q$ denotes a theoretical joint distribution, the fitting criterion is
\begin{equation}
\mathrm{FitKL}(Q)=D_{\mathrm{KL}}(\widehat\rho\,\|\,Q)
=\sum_a \widehat\rho(a)\log\frac{\widehat\rho(a)}{Q(a)}.
\label{eq:fitkl-main}
\end{equation}
Lower values indicate better agreement with the empirical joint distribution.  The main human benchmark is the Selten--Chmura dataset of completely mixed $2\times2$ games.  The main LLM benchmark uses one-shot weighted rock--paper--scissors games with shared public signals.  The earlier smoothed fictitious-play benchmark is reported in Appendix~\ref{appendix:synthetic-details}; we use it as a controlled diagnostic rather than as the main empirical claim.

\subsection{Bootstrap confidence intervals}
\label{subsec:bootstrap-ci}

The two empirical settings have different sampling units, so we use different nonparametric bootstrap schemes.
For the Selten--Chmura human data, the independent unit is a subject group.  For each game $g\in\{1,\ldots,6\}$, the public spreadsheet gives $12$ independent group-level empirical joint distributions, which we write as
\begin{equation}
\widehat\rho_{g,1},\ldots,\widehat\rho_{g,12}\in\Delta(\{U,D\}\times\{L,R\}).
\end{equation}
For bootstrap replicate $b$, we sample indices $J_{g,1}^{(b)},\ldots,J_{g,12}^{(b)}$ independently with replacement from $\{1,\ldots,12\}$ and form
\begin{equation}
\widehat\rho_g^{*(b)}
=\frac{1}{12}\sum_{r=1}^{12}\widehat\rho_{g,J_{g,r}^{(b)}}.
\label{eq:selten-bootstrap-rho}
\end{equation}
For a fixed fitted model prediction $Q_{g,m}$, the bootstrap KL for game $g$ and model $m$ is
\begin{equation}
K_{g,m}^{*(b)}=D_{\mathrm{KL}}\!\left(\widehat\rho_g^{*(b)}\,\|\,Q_{g,m}\right).
\label{eq:selten-bootstrap-game-kl}
\end{equation}
The mean-over-games bootstrap statistic reported in the main table is
\begin{equation}
\overline K_{m}^{*(b)}=\frac{1}{6}\sum_{g=1}^6 K_{g,m}^{*(b)}.
\label{eq:selten-bootstrap-mean-kl}
\end{equation}
Repeating this for $B=2000$ replicates gives a bootstrap distribution of $\overline K_m^*$.  We report the bootstrap mean and the percentile interval
\begin{equation}
\left[Q_{2.5\%}\!\left(\overline K_m^*\right),\ Q_{97.5\%}\!\left(\overline K_m^*\right)\right].
\end{equation}
The fitted model predictions $Q_{g,m}$ are held fixed inside the bootstrap.  Thus the interval measures uncertainty from finite subject-group sampling, not uncertainty from refitting the model on every bootstrap replicate.

For the LLM data, the independent unit is one one-shot match.  If $x_1,\ldots,x_N\in A\times A$ are the observed action pairs, a bootstrap replicate samples $N$ rows with replacement and constructs
\begin{equation}
\widehat p^{*(b)}(a_1,a_2)
=\frac{1}{N}\sum_{t=1}^{N}\mathbf 1\{x_{I_t^{(b)}}=(a_1,a_2)\},
\label{eq:llm-bootstrap-rho}
\end{equation}
where $I_1^{(b)},\ldots,I_N^{(b)}$ are sampled uniformly from $\{1,\ldots,N\}$.  Equivalently, for the round-robin experiments we may draw a multinomial count vector $X^{(b)}\sim\mathrm{Mult}(N,\widehat p)$ and set $\widehat p^{*(b)}=X^{(b)}/N$.  For each fixed fitted LLM model prediction $Q_m$, we compute
\begin{equation}
K_m^{*(b)}=D_{\mathrm{KL}}\!\left(\widehat p^{*(b)}\,\|\,Q_m\right)
\label{eq:llm-bootstrap-kl}
\end{equation}
and again report percentile confidence intervals.  This bootstrap is different from the Selten--Chmura one because the LLM data contain raw one-shot match rows, whereas the Selten--Chmura spreadsheet releases only group-level empirical joint distributions.

\subsection{Selten--Chmura human benchmark}
\label{subsec:selten-human-results}

The Selten--Chmura data consist of repeated random-matching population play in $2\times2$ games.  We focus on the first six constant-sum games.  For each game $g\in\{1,\ldots,6\}$, there are $12$ independent subject groups.  Each group contains four player-1 subjects and four player-2 subjects, matched randomly over $200$ periods, so each group contributes $800$ realized action pairs.  We aggregate the full-horizon counts across the $12$ independent groups and form
\begin{equation}
\widehat\rho_g(a_1,a_2)
=
\frac{\sum_j C^{(200)}_{g,j}(a_1,a_2)}{\sum_j\sum_{a_1',a_2'} C^{(200)}_{g,j}(a_1',a_2')}.
\label{eq:empirical-joint-main}
\end{equation}
For each game and each CQRE family, relaxation parameters are chosen by an in-sample grid search over the empirical joint distribution for that game.  For logit QRE, the inverse-temperature parameter is also fit separately for each game.

\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
Game & Nash & Exact CQRE & Logit QRE product & CQRE scalar & CQRE per-player & CQRE per-action \\
\midrule
1 & 0.1910 & 0.1910 & 0.0183 & 0.0056 & 0.0019 & 0.0019 \\
2 & 0.0947 & 0.0947 & 0.0053 & 0.0068 & 0.0051 & 0.0051 \\
3 & 0.0952 & 0.0952 & 0.0002 & 0.0356 & 0.0347 & 0.0270 \\
4 & 0.0344 & 0.0344 & 0.0002 & 0.0147 & 0.0147 & 0.0102 \\
5 & 0.0132 & 0.0132 & 0.0011 & 0.0062 & 0.0044 & 0.0035 \\
6 & 0.0039 & 0.0039 & 0.0021 & 0.0017 & 0.0008 & 0.0008 \\
\midrule
Mean & 0.0721 & 0.0721 & 0.0046 & 0.0118 & 0.0103 & 0.0081 \\
\bottomrule
\end{tabular}
\caption{Per-game fitting on Selten--Chmura constant-sum games $1$--$6$: $D_{\mathrm{KL}}(\widehat\rho_g\,\|\,Q_g)$. Lower is better.}
\label{tab:first6-main-fit}
\end{table*}

\begin{table*}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
Model & Full-data mean KL & Bootstrap mean KL & 95\% CI \\
\midrule
Logit QRE product & 0.0046 & 0.0061 & $[0.0032,\,0.0099]$ \\
CQRE per-action & 0.0081 & 0.0095 & $[0.0062,\,0.0137]$ \\
CQRE per-player & 0.0103 & 0.0117 & $[0.0079,\,0.0162]$ \\
CQRE scalar & 0.0118 & 0.0132 & $[0.0095,\,0.0177]$ \\
Nash & 0.0721 & 0.0738 & $[0.0600,\,0.0903]$ \\
Exact CQRE & 0.0721 & 0.0738 & $[0.0600,\,0.0903]$ \\
\bottomrule
\end{tabular}
\caption{Bootstrap confidence intervals for mean KL on Selten--Chmura games $1$--$6$.  Each bootstrap replicate resamples the $12$ independent group-level empirical joint distributions within each game, averages them to form a new empirical game-level joint, and recomputes the KL to fixed fitted model predictions.}
\label{tab:first6-mean-ci}
\end{table*}

Table~\ref{tab:first6-main-fit} shows that the exact CQRE predictor coincides numerically with the mixed Nash product in these six constant-sum games.  Both are much worse than the relaxed and logit-QRE benchmarks.  Relaxation improves CQRE substantially in every game, and the per-action family gives the best average CQRE fit.  Table~\ref{tab:first6-mean-ci} qualifies this mean comparison with uncertainty estimates.  Logit QRE has the lowest full-data mean KL, but the confidence interval for per-action CQRE overlaps with that of logit QRE.  Thus the human data support the conservative claim that relaxed CQRE gives a close empirical fit and is clearly better than exact CE/Nash, while logit QRE remains a very strong product-form benchmark.

\subsection{One-shot Qwen weighted-RPS benchmark}
\label{subsec:llm-rps-results}

As a local LLM pilot, we generated one-shot weighted rock--paper--scissors data using Qwen2.5-3B-Instruct-4bit.  The game uses action order $(R,P,S)$ and payoffs
\begin{equation}
U_1=\begin{pmatrix}
2 & 1 & 4\\
3 & 2 & 1\\
0 & 3 & 2
\end{pmatrix},
\qquad
U_2=\begin{pmatrix}
2 & 3 & 0\\
1 & 2 & 3\\
4 & 1 & 2
\end{pmatrix}.
\label{eq:weighted-rps-payoff-main}
\end{equation}
The dataset consists of $200$ independent one-shot matches.  Both players observe the full payoff matrix, including both players' payoffs, and the move is simultaneous.  We use a shared-signal condition: both prompts include the same public signal for the round, but no history is provided and each match starts from a fresh context.  The empirical target $\widehat\rho_{\mathrm{LLM}}$ is the empirical joint distribution of the resulting action pairs.  Bootstrap confidence intervals are computed by resampling the $200$ one-shot match rows with replacement.

\begin{table*}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
Model & Full-data KL & Bootstrap mean KL & 95\% CI \\
\midrule
CQRE per-action & 0.3518 & 0.3692 & $[0.2890,\,0.4601]$ \\
Logit QRE product & 0.3530 & 0.3702 & $[0.2925,\,0.4556]$ \\
CQRE scalar & 0.3625 & 0.3798 & $[0.3014,\,0.4688]$ \\
CQRE per-player & 0.3625 & 0.3798 & $[0.3014,\,0.4688]$ \\
Nash & 0.7646 & 0.7813 & $[0.6581,\,0.9090]$ \\
Exact CQRE & 0.7646 & 0.7813 & $[0.6581,\,0.9090]$ \\
\bottomrule
\end{tabular}
\caption{One-shot Qwen weighted-RPS fitting results under the shared-signal condition.  The empirical joint is computed from $200$ independent Qwen2.5-3B-Instruct-4bit self-play matches. Lower KL is better.}
\label{tab:llm-rps-ci}
\end{table*}

Table~\ref{tab:llm-rps-ci} shows a qualitatively similar pattern: Nash and exact CQRE are too rigid, while QRE and relaxed CQRE fit the LLM empirical joint much better.  In this sample, per-action CQRE has the smallest full-data KL, but the confidence intervals for per-action CQRE and logit QRE overlap almost completely.  This pilot therefore motivates a larger LLM experiment with more models and model pairs.

\subsection{Frontier GPT round-robin benchmark}
\label{subsec:gpt-roundrobin-results}

We next study one-shot weighted-RPS play across six OpenAI GPT deployments: \textsf{gpt-4o}, \textsf{gpt-4o-mini}, \textsf{gpt-4.1}, \textsf{gpt-4.1-mini}, \textsf{gpt-5}, and \textsf{gpt-5-mini}.  For each unordered model pair, we generate $N=200$ independent one-shot matches using the same payoff matrix in~\eqref{eq:weighted-rps-payoff-main}.  The assignment of the two models to row and column roles is randomized across matches; the displayed action labels are randomly permuted; both players see the full permuted payoff matrix and a shared public signal; and each match is generated from a fresh prompt.  We completed $20$ of the $21$ unordered pairs; the \textsf{gpt-5} self-play pair timed out and is omitted.

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{cqre_vs_qre_scatter.pdf}
\caption{Logit QRE vs. CQRE per-action.}
\label{fig:gpt-qre-scatter}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{fit_model_delta_bar.pdf}
\caption{KL reduction from CQRE per-action.}
\label{fig:gpt-delta-bar}
\end{subfigure}
\caption{Frontier GPT round-robin results on weighted RPS.  Left: each point is one model pair, with KL to logit QRE on the horizontal axis and KL to CQRE per-action on the vertical axis.  Points below the diagonal are better fit by CQRE per-action.  Right: per-pair reduction in KL obtained by CQRE per-action relative to Nash and logit QRE.}
\label{fig:gpt-roundrobin-main}
\end{figure*}

The round-robin results sharpen the LLM picture.  CQRE per-action weakly improves on Nash and exact CQRE on every completed pair.  It also weakly dominates the nested CQRE scalar and per-player families by construction of the relaxation grid.  Against logit QRE, CQRE per-action has a smaller point-estimate KL on $11$ of the $20$ completed pairs.  On the remaining pairs, the difference is small and within bootstrap uncertainty.  The largest improvement over logit QRE occurs in the \textsf{gpt-4o} self-play pair, where CQRE per-action reduces KL by approximately $0.14$ nats.  Figure~\ref{fig:gpt-roundrobin-main} shows that the advantage of per-action CQRE is concentrated in high-deviation regimes such as self-play and intra-family pairs, while many cross-model pairs lie close to the QRE--CQRE diagonal.

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{cqre_per_action_bar.pdf}
\caption{Pairs sorted by CQRE per-action KL.}
\label{fig:gpt-cqre-bar}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{cqre_self_vs_cross.pdf}
\caption{Self-play vs. cross-model pairs.}
\label{fig:gpt-self-cross}
\end{subfigure}
\caption{Additional views of the GPT round-robin.  Self-play pairs generally have larger KL to CQRE per-action than cross-model pairs, suggesting that same-model interactions generate more concentrated and harder-to-fit joint behavior.}
\label{fig:gpt-roundrobin-secondary}
\end{figure*}

The GPT round-robin strengthens the interpretation of CQRE as a flexible empirical benchmark for LLM play.  The key point is not that CQRE per-action always decisively beats logit QRE; rather, it is never clearly worse in these experiments, it captures model-pair regimes where product-form QRE struggles, and it uniformly improves over exact CE/Nash.

\subsection{Summary of empirical findings}
\label{subsec:empirical-summary}

Across human and LLM benchmarks, exact CE/Nash is consistently too rigid.  Relaxed CQRE substantially improves fit by allowing approximate obedience.  On human Selten--Chmura data, logit QRE has the best mean KL but per-action CQRE is close with overlapping confidence intervals.  On local Qwen weighted-RPS data, per-action CQRE is slightly best in the observed sample but statistically tied with logit QRE.  On the larger GPT round-robin, per-action CQRE weakly dominates Nash and nested CQRE variants on every completed pair and is competitive with or better than logit QRE, especially in self-play and high-deviation model-pair regimes.  These results support a conservative but useful conclusion: CQRE is not a universal replacement for product-form QRE, but it is a strong relaxed-obedience joint-distribution benchmark for empirical strategic behavior.


==> sections/00_abstract.tex <==
\begin{abstract}
  We introduce \emph{correlated quantal response equilibrium with per-action slack}
  (CQRE-pa), the unique maximum-entropy joint distribution satisfying per-action
  exploitability constraints in a finite normal-form game, as a new equilibrium notion
  for studying human and language-model strategic behavior.  We provide two estimators:
  a seven-point slack-grid procedure and a rigorous continuous bilevel method. We also contribute a reproducible dataset containing 201,600 accepted one-shot decisions from six OpenAI model deployments across all 12 presentations of the six
  Selten--Chmura $2{\times}2$ game families. Combined with historical human frequencies, the dataset supports 588 standardized targets---432 AI--AI, 144 directional human--AI, and 12 human--human,
  with $n=200$ each---and provides a resource for future research on comparative human--AI strategic behavior.

  Three findings emerge.  (i) Continuous optimization improves 304 of 576 AI-involving CQRE-pa fits and worsens none.  (ii) In the all-12 same-target analysis, continuous CQRE-pa significantly
  outperforms extended-domain Logit-QRE on both AI--AI and genuine human--human play.
  On the 432 AI--AI targets, mean KL has a $3.0\%$
  reduction with paired improvement. On the 12 human--human targets, mean KL has a $56.9\%$ reduction.  Across all 588 targets, CQRE-pa retains a significant target-weighted advantage. (iii) Under the frozen-grid optimization, CQRE-pa strictly wins $111/147=75.5\%$ of two-player paired tests and $55/56$ symmetric three-player triplets; Logit-QRE never strictly wins on any three-player triplet.  We claim that this new notion is a better fit for describing human-human and AI-AI joint behavior for strategic games.
  \end{abstract}

% =====================================================================


==> sections/01_introduction.tex <==
\section{Introduction}
% =====================================================================

Large language models are increasingly deployed as autonomous strategic agents, raising the
basic empirical question: \emph{which equilibrium notion best describes their joint play?}
Classical (mixed) Nash equilibrium~\citep{nash1951noncoop} is too rigid for noisy agents. Quantal response
equilibrium~\citep{mckelvey1995qre,goeree2005regular} relaxes best response via a softmax
with a single inverse-temperature per player, and is the standard relaxation for human
experimental data~\citep{selten2008stationary}. Correlated
equilibrium~\citep{aumann1974subjectivity,aumann1987correlated} permits joint recommendations
but no per-action mistakes.

 Our empirical account begins with human--human play.  The Selten--Chmura observations are within-group joint play and provide the
  most direct behavioral benchmark, but they are a fixed, limited laboratory data
  set rather than a repeatable collection pipeline.  This motivates the AI
  extension: six models supply one-shot choices in all 12 presentations of the six payoff-translation-equivalent strategic families, allowing systematic AI--AI (AAI) and directional human--AI (HAI) comparisons while retaining the original human frequencies.  The paired-seven AAI targets combine outcome-blind archival allocations with fresh paired calls, which resembles human--human (HH) data; the HAI (Human vs AI, directional) targets are marginal products, the constructions are not observed human--AI interaction, and the product targets cannot identify within-play correlation.

Recent work~{~\citep{akata2023playing,lore2024strategicllms,pezeshkpour2024llmsensitivity,zheng2024llmrobustchoice}} shows that LLM agents exhibit two patterns that neither classical relaxation captures well:
(i)~\emph{action-label bias}---when the same payoff matrix is relabeled, LLMs systematically
prefer specific labels (e.g.\ ``A''), and (ii)~\emph{collapse:} frontier models often
concentrate $\ge 99\%$ of their probability on a single action profile.  A scalar
inverse-temperature cannot emulate the behavior in (i), and a single $\beta$ asymptote cannot interpolate
between (ii) and the more diffuse play of weaker models in the same game.  We propose a
relaxation that handles both, namely, maximum-entropy correlated equilibrium with one slack
\emph{per (player, action) pair}.


\begin{figure}[!t]
\centering
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{0pt}
\begin{adjustbox}{center,max width=1.25\textwidth}
\includegraphics[width=1.25\textwidth]{pipeline.png}
\end{adjustbox}
\caption{\small End-to-end experimental pipeline. Empirical joint play is collected from two sources.
Humans: the 6 unique-mixed-Nash $2\times2$ games of Selten--Chmura (12 student groups per game).
LLMs: a round-robin among 6 OpenAI deployments (gpt-4o, gpt-4o-mini,
gpt-4.1, gpt-4.1-mini, gpt-5, gpt-5-mini), where every (un)ordered tuple
of deployments plays $N{=}200$ matches per game, covering 7 two-player games
(strongly-monotone with action size $n\in\{3,5,7\}$ and rank-$r$ asymmetric for
$r\in\{1,\ldots,4\}$; 21 dyads per game) and 2 three-player games (\texttt{jordan\_3p2a},
whose cyclic role asymmetry yields $6^3{=}216$ ordered triples, and the fully symmetric
\texttt{sm\_3p3a} with $\binom{6+3-1}{3}{=}56$ unordered multisets). For each (game, pair)
we fit six equilibrium notions to the observed joint $\hat p$ by minimizing
$\KL(\hat p\,\Vert\,p^\star)$; multinomial bootstrap ($B{=}1000$) yields a 95\% CI per notion,
and the paired difference $\Delta=\KL_{\text{CQRE-pa}}-\KL_{\text{Logit-QRE}}$ delivers a CI-based
per-(game, pair) result. Total: 541 headline fits, all bit-perfectly reproducible
(Section~\ref{sec:reproducibility-main}); the appendix replicates every comparison under TV, $L_2$, and Rényi-$1/2$ distances. The all-12 extension uses a sealed 115,200-choice archive and 86,400 fresh paired calls (201,600 accepted AI decisions in the paired-seven corpus) to form 588 separately fitted targets.}
\label{fig:pipeline}
\end{figure}

We define CQRE-pa as the maximum-entropy correlated strategy in a closed convex polytope parameterized by a nonnegative slack vector $\gamma\in\Real_+^{2n}$, and prove existence,
  uniqueness, and an exponential-family closed form in Section~\ref{sec:cqre}. Section~\ref{sec:compute} specifies the convex solver, the discrete slack grid and the continuous
  bilevel outer-slack estimator, the five comparison notions (mixed Nash, Logit-QRE, exact CQRE, scalar CQRE, per-player CQRE), and the paired bootstrap test. Section~\ref{sec:empirical} reports the empirical evaluation on three independent corpora: on the Selten--Chmura $2\times2$ human dataset (6 games, 12 subject-groups per
  game), CQRE-pa and Logit-QRE are the two closest-fitting notions, with overlapping
  marginal intervals in all six games; under the discrete grid search, CQRE-pa
  strictly wins $111/147=75.5\%$ of paired tests in the 7-game multi-LLM tournament
  and $55/56$ symmetric \texttt{sm\_3p3a} three-player triplets, while Logit-QRE
  never strictly wins a three-player triplet. The new all-12 Selten extension contributes
  a reproducible dataset of 201,600 accepted one-shot AI decisions and supports 588
  standardized targets. The bounded continuous optimizer improves 304 of 576
  AI-involving CQRE-pa fits and worsens none. In the same-target comparison with
  extended-domain Logit-QRE, continuous CQRE-pa reduces mean KL by $3.0\%$ on
  432 AI--AI targets and by $56.9\%$ on 12 human--human targets, while
  retaining a significant target-weighted advantage across all 588 targets. These
  results support CQRE-pa as the better-fitting aggregate benchmark for AI--AI and
  human--human joint behavior in the all-12 evaluation.
Section~\ref{sec:discussion} discusses the implications, population differences, and
  limitations. Appendices~\ref{app:proofs}--\ref{app:solver} provide proofs, additional
  distance metrics, full confidence intervals, robustness analyses, reproducibility
  audits, and details of the continuous outer optimizer.

\textbf{RJ: This is a very unusually dense intro. An intro has to tell a story that another person can understand, not bury the reader in detail.}

\begin{remark}
\textbf{Reproducibility:} All numerical results reproduce bit-perfect on $541$ fits
under a locked environment---see  Section~\ref{sec:reproducibility-main} and 
Appendix~\ref{app:reproducibility} for details.
\end{remark}





==> sections/02_correlated_quantal_response_equilibrium.tex <==
\section{Correlated Quantal Response Equilibrium}
\label{sec:cqre}
% =====================================================================

\textbf{RJ: This needs some context. Given two players, suppose their payoffs are given by blah blah... is it AI-generated?}

Let $A_1, A_2$ be finite action sets and $U_1, U_2 : A_1\times A_2\to\Real$ bounded
utilities.  Denote by $\rho$ a joint distribution from $\Simplex(A_1\times A_2)$.

\textbf{RJ: there is no motivation before the def.}

\begin{definition}[Slack-relaxed obedience polytope]
\label{def:feasible}
For a nonnegative slack vector $\gamma
  :=
  \bigl((\gamma_{1,a})_{a\in A_1},
        (\gamma_{2,a})_{a\in A_2}\bigr)
  \in\Real_+^{|A_1|+|A_2|}$,
$K_\gamma\subseteq\Simplex(A_1\times A_2)$ is the set of joint distributions satisfying the 
per-action recommendation deviation bounds
\begin{align}
\textstyle\sum_{a_2}\rho(a_1,a_2)\bigl(U_1(\widetilde a_1,a_2)-U_1(a_1,a_2)\bigr)\;&\le\;\gamma_{1,a_1},\ \ \forall\,a_1,\,\widetilde a_1\neq a_1,\label{eq:dev1}\\
\textstyle\sum_{a_1}\rho(a_1,a_2)\bigl(U_2(a_1,\widetilde a_2)-U_2(a_1,a_2)\bigr)\;&\le\;\gamma_{2,a_2},\ \ \forall\,a_2,\,\widetilde a_2\neq a_2.\label{eq:dev2}
\end{align}
\end{definition}

% \sout{\noindent Setting $\gamma=0$ recovers the classical correlated-equilibrium
% polytope~\citep{aumann1987correlated}; sending the smallest entry of $\gamma$ to $+\infty$
% recovers all of $\Simplex(A_1\times A_2)$.}

The two endpoints recover familiar limits.  When $\gamma=0$, every per-(player, action)
obedience inequality must bind weakly, so $K_0$ coincides with the classical
correlated-equilibrium polytope \citep{aumann1987correlated} and $\rho^\star_0$ is the
maximum-entropy correlated equilibrium \citep{jaynes1957information,hart2000simple}.   At the
other extreme, as $\min_{k,a}\gamma_{k,a}\to\infty$ every constraint becomes vacuous,
$K_\gamma=\Simplex(A_1\times A_2)$, and $\rho^\star_\gamma$ converges to the uniform
distribution on $A_1 \times A_2$. For intermediate $\gamma$, the maximum-entropy point interpolates between these
two extremes. Because $\gamma$ is indexed by every (player, action) pair, the relaxation can be tightened or loosened on a per-action basis, which is the flexibility needed to represent LLM action-label asymmetry — a single 
$\beta$ in Logit-QRE cannot.

\textbf{RJ: QRE needs to be defined before, and one should motivate why it is not adequate.}

\begin{definition}[CQRE-pa]
\label{def:cqre}
For fixed $\gamma\ge 0$, the \emph{per-action correlated quantal response equilibrium} is
\begin{equation}
\rho_\gamma^\star\;\in\;\argmin_{\rho\in K_\gamma}\;\sum_{(a_1,a_2)}\rho(a_1,a_2)\log\rho(a_1,a_2).
\label{eq:cqre}
\end{equation}
\end{definition}
 
\noindent At $\gamma=0$ this selects the maximum-entropy correlated
equilibrium~\citep{jaynes1957information,hart2000simple}; positive slacks interpolate
continuously towards the uniform joint.

\begin{theorem}[Existence and uniqueness]
\label{thm:exists}
For finite $A_1, A_2$, bounded $U_1, U_2$, and any $\gamma\ge 0$, problem
\eqref{eq:cqre} admits exactly one optimizer.
\end{theorem}

\begin{proof}[Proof]
Any mixed Nash $(\sigma_1,\sigma_2)$ yields a product joint $\bar\rho\in K_\gamma$ (the
deviation slack is $\le 0$ for any best-response action).  $K_\gamma$ is compact and the
negative Shannon entropy is strictly convex on the simplex, so the minimizer exists and is
unique.  Full proof can be found in Appendix~\ref{app:proofs}.
\end{proof}

\textbf{RJ: needs a comment on implication.}

\begin{proposition}[Exponential-family form]
\label{prop:exp}

If $\rho_\gamma^\star$ has full support, then it satisfies
\begin{equation}
\rho^\star(a_1,a_2)\;\propto\;\exp\!\Big(\textstyle\sum_{\widetilde a_1}\!\lambda_{1,a_1,\widetilde a_1}\Delta U_{1}(a_1,\widetilde a_1;a_2)+\sum_{\widetilde a_2}\!\lambda_{2,a_2,\widetilde a_2}\Delta U_{2}(a_2,\widetilde a_2;a_1)\Big),
\label{eq:gibbs}
\end{equation}
where $\Delta U_k(a,\widetilde a;a_{-k}):=U_k(a,a_{-k})-U_k(\widetilde a,a_{-k})$ is the
deviation payoff and $\lambda\ge 0$ are the KKT multipliers of the active deviation
inequalities.
\end{proposition}



The exponential form \eqref{eq:gibbs} makes the connection to QRE explicit: Logit-QRE uses a single $\beta_k$ per player and forces $\rho=\sigma_1\otimes\sigma_2$
to be a product, whereas CQRE-pa permits per-(player, action) slacks $\gamma_{k,a}$ and
carries across-player correlation.  For $N$ players we replace the joint with
$\rho\in\Simplex(\prod_k A_k)$, retain one slack per (player, action) ($\gamma_{k,a}$), and
\eqref{eq:gibbs} generalizes by summing across all players $k$.

% =====================================================================


==> sections/03_computation_and_comparison_notions.tex <==
\section{Computation and Comparison Notions}
\label{sec:compute}
% =====================================================================
%We retain $K_\gamma$ and $\rho_\gamma^\star$ from Section~\ref{sec:cqre}. For the multiplayer extension, 
Let $\mathcal P$ be
the finite player set and let
$\mathcal X:=\prod_{k\in\mathcal P}A_k$ be the set of joint action profiles, with
$d_{\mathcal X}:=|\mathcal X|=\prod_{k\in\mathcal P}|A_k|$. For
$x=(x_k)_{k\in\mathcal P}\in\mathcal X$, $x_{-k}$ denotes the actions of all
players other than $k$, and $U_k(a,x_{-k})$ is player $k$'s payoff when
player $k$ chooses $a$ and the other players choose $x_{-k}$.

Index the obedience inequalities by
$
\mathcal R
:=
\{(k,a,\widetilde a):k\in\mathcal P,\ a,\widetilde a\in A_k,
\ \widetilde a\ne a\},
\qquad
d_{\mathcal R}:=|\mathcal R|
=\sum_{k\in\mathcal P}|A_k|(|A_k|-1),
$
and the player-action slack coordinates by
$\mathcal I:=\{(k,a):k\in\mathcal P,\ a\in A_k\}$, with
$d_{\mathrm{pa}}:=|\mathcal I|=\sum_{k\in\mathcal P}|A_k|$.
After fixing orderings of $\mathcal X$, $\mathcal R$, and $\mathcal I$,
write $\rho=(\rho_x)_{x\in\mathcal X}\in\Real^{d_{\mathcal X}}$ and
$\gamma=(\gamma_{k,a})_{(k,a)\in\mathcal I}\in\Real_+^{d_{\mathrm{pa}}}$.

Define the obedience matrix
$A\in\Real^{d_{\mathcal R}\times d_{\mathcal X}}$ and per-action
replication matrix
$D_{\mathrm{pa}}\in\{0,1\}^{d_{\mathcal R}\times d_{\mathrm{pa}}}$ by
$$
A_{(k,a,\widetilde a),x}
:=
\mathbf1\{x_k=a\}
\bigl[U_k(\widetilde a,x_{-k})-U_k(a,x_{-k})\bigr],
\qquad
(D_{\mathrm{pa}})_{(k,a,\widetilde a),(\ell,c)}
:=\mathbf1\{k=\ell,\ a=c\}.
$$
Thus, for $s=(k,a,\widetilde a)\in\mathcal R$,
$$
(A\rho)_s
=\sum_{x_{-k}}\rho(a,x_{-k})
\bigl[U_k(\widetilde a,x_{-k})-U_k(a,x_{-k})\bigr],
\qquad
(D_{\mathrm{pa}}\gamma)_s=\gamma_{k,a}.
$$
Writing $\mathbf1_{d_{\mathcal X}}$ for the all-ones vector, the
multiplayer version of Definition~\ref{def:feasible} is therefore
\begin{equation}
K_\gamma
=
\left\{
\rho\in\Real_+^{d_{\mathcal X}}:
\mathbf1_{d_{\mathcal X}}^\top\rho=1,
\quad A\rho\le D_{\mathrm{pa}}\gamma
\right\}.
\label{eq:matrix-feasible-set}
\end{equation}



\begin{lemma}[Convexity of the inner program]
\label{lem:inner-convex}
For any fixed $\gamma\in\Real_+^{d_{\mathrm{pa}}}$, the multiplayer
extension of problem~\eqref{eq:cqre} is a convex program in $\rho$ with
$d_{\mathcal X}$ variables and $d_{\mathcal R}$ linear obedience
inequalities. Its optimizer is unique.
\end{lemma}

% \begin{lemma}[Convexity of the inner program]
% \label{lem:inner-convex}
% For any fixed $\gamma\ge 0$, problem~\eqref{eq:cqre} is a convex program in $\rho$ with $\prod_k |A_k|$ variables and $\sum_k |A_k|(|A_k|-1)$ linear inequality constraints.
% \end{lemma}

\begin{definition}[Slack parameterizations]
\label{def:slack-params}
We consider three nested parameterizations. Let
$m\in\{\mathrm{sc},\mathrm{pp},\mathrm{pa}\}$ denote the scalar,
per-player, or per-action specification, respectively, and let
$$
d_{\mathrm{sc}}:=1,
\qquad
d_{\mathrm{pp}}:=|\mathcal P|,
\qquad
d_{\mathrm{pa}}:=\sum_{k\in\mathcal P}|A_k|.
$$
For free coordinates $\theta\in\Real_+^{d_m}$, define the full
per-action slack vector $\gamma_m(\theta)\in\Real_+^{d_{\mathrm{pa}}}$ by
$$
[\gamma_m(\theta)]_{k,a}
:=
\begin{cases}
\theta_1, & m=\mathrm{sc},\\
\theta_k, & m=\mathrm{pp},\\
\theta_{k,a}, & m=\mathrm{pa}.
\end{cases}
$$
\textbf{RJ: it might be better to use sub and superscripts for sc and pp, else confusing.}

Thus the scalar specification has one common slack, the per-player
specification has one slack for each player, and the per-action specification
has one slack for each player-action pair. We refer to the last specification
as \emph{CQRE-pa}. Let
$D_m\in\{0,1\}^{d_{\mathcal R}\times d_m}$ be the corresponding
replication matrix, defined by
$$
(D_m\theta)_{(k,a,\widetilde a)}
:=[\gamma_m(\theta)]_{k,a}.
$$
Then
$$
K_m(\theta)
:=K_{\gamma_m(\theta)}
=\left\{\rho\in\Real_+^{d_{\mathcal X}}:
\mathbf1_{d_{\mathcal X}}^\top\rho=1,
\ A\rho\le D_m\theta\right\},
\qquad
\rho_m^\star(\theta):=\rho_{\gamma_m(\theta)}^\star.
$$
\end{definition}

Let $\hat p=(\hat p_x)_{x\in\mathcal X}\in\Simplex(\mathcal X)$ denote
the empirical distribution. For specification $m$, the empirical
Kullback--Leibler (KL) loss is
$$
L_m(\theta)
:=\KL\!\left(\hat p\,\middle\|\,\rho_m^\star(\theta)\right),
$$
which is optimized over the free slack coordinates $\theta$.




\begin{lemma}[Nesting]
\label{lem:nesting}
Every $\rho_m^\star(\theta)$ achievable under the scalar parameterization is also achievable under per-player, and every solution
achievable under the per-player parameterization is also achievable under the per-action parameterization. Hence the minimum empirical KL divergence is non-increasing in the flexibility of the parameterization.
% and every $\rho^\star_\gamma$ achievable under per-player is also achievable under per-action. Hence $\min_\gamma \KL(\hat p \,\|\, \rho^\star_\gamma)$ is non-increasing in the flexibility of the parameterization.
\end{lemma}


  \begin{remark}
  Lemma~\ref{lem:nesting} guarantees only that training-
  time KL is
  non-increasing as the slack parameterization becomes
  more flexible. The
  point estimates in Table~\ref{tab:selten} are
  consistent with this ordering:
  continuous CQRE-pa has weakly lower KL than the grid-
  fitted scalar and
  per-player specifications in every game. 
  \end{remark}




% The empirical loss is $\KL(\hat p \,\|\, \rho^\star_\gamma)$, optimized over the slack vector $\gamma$.



This is a bilevel estimation problem, not a joint fit of $(\rho,\theta)$:
the outer procedure selects $\theta$, the inner entropy program uniquely
selects $\rho_m^\star(\theta)$, and the outer criterion is $L_m(\theta)$.
Minimizing KL directly over a merely feasible pair $(\rho,\theta)$ would drop
the defining requirement that $\rho$ be the maximum-entropy solution for its
slack. Also, increasing slack need not lower $L_m$: after the obedience
constraints become redundant, the inner solution is uniform rather than the
empirical target.

  Our estimator tries to optimize slack over a compact domain. For
  each per-action coordinate, let
  \[
  h_{k,a}=\max\!\left\{0,\max_{\widetilde a\ne a}\max_{a_{-k}}
   [U_k(\widetilde a,a_{-k})-U_k(a,a_{-k})]\right\}.
  \]
Any larger value of $\gamma_{k,a}$ is redundant on the simplex, so
$\gamma\in\prod_{(k,a)\in\mathcal I}[0,h_{k,a}]$ provides a representative
of every attainable CQRE distribution. The payoff normalization described in
Appendix~\ref{app:solver} gives $h_{k,a}\le1$. The scalar, per-player, and
per-action optimization domains are
therefore
$$
\Theta_{\mathrm{sc}}=[0,1],
\qquad
\Theta_{\mathrm{pp}}=[0,1]^{d_{\mathrm{pp}}},
\qquad
\Theta_{\mathrm{pa}}
=\prod_{(k,a)\in\mathcal I}[0,h_{k,a}],
$$
respectively. Appendix~\ref{app:solver} proves that
$\theta\mapsto K_m(\theta)$ is a continuous compact-valued correspondence. Hence, by Berge's Maximum Theorem~\citep[Page 116]{berge1963espaces}, $\rho_m^\star(\theta)$ is continuous, and so, a minimum for the continuous function $L_m$ is lower semicontinuous and attains a finite minimum on each domain $\Theta_m$. It is continuous wherever $\rho_{m,x}^\star(\theta)>0$ for every $x$ with $\hat p_x>0$.
  %When $\rho^\star_\gamma$ is also differentiable in $\gamma$ we 

We next define the quantities used to differentiate the inner
Karush--Kuhn--Tucker (KKT) system. Fix $m$ and $\theta$, write
$\rho^\star:=\rho_m^\star(\theta)$, and let
$$
S
:=\{s\in\mathcal R:A_s\rho^\star=(D_m\theta)_s\}
$$
be the set of binding obedience inequalities, where $A_s$ denotes row $s$ of
$A$. Let $A_S\in\Real^{|S|\times d_{\mathcal X}}$ and
$D_{m,S}\in\Real^{|S|\times d_m}$ contain the rows of $A$ and $D_m$
indexed by $S$, and define
$$
C_S
:=
\begin{bmatrix}
\mathbf1_{d_{\mathcal X}}^\top\\
A_S
\end{bmatrix}
\in\Real^{(1+|S|)\times d_{\mathcal X}},
\qquad
G_{m,S}
:=
\begin{bmatrix}
0_{1\times d_m}\\
D_{m,S}
\end{bmatrix}
\in\Real^{(1+|S|)\times d_m},
$$
and
$W:=\operatorname{diag}(\rho^\star)
\in\Real^{d_{\mathcal X}\times d_{\mathcal X}}$.
On a neighborhood in which $S$ is unchanged, suppose that
$\rho^\star$ has full support, the numerical probability floor is inactive,
the inactive obedience inequalities are strict, the active multipliers are
positive, and $C_S$ has full row rank. Then
differentiating the KKT system gives
\begin{align}
J_m:=\frac{\partial\rho_m^\star}{\partial\theta}
&=WC_S^\top(C_SWC_S^\top)^{-1}G_{m,S}
\in\Real^{d_{\mathcal X}\times d_m},
\label{eq:continuous-jacobian}\\
\nabla_\theta L_m
&=-J_m^\top(\hat p\oslash\rho^\star)
\in\Real^{d_m},
\label{eq:continuous-hypergradient}
\end{align}
where $\oslash$ denotes entrywise division. The derivation and the precise
regularity conditions are given in
Proposition~\ref{prop:continuous-outer-derivative} of
Appendix~\ref{app:solver}.

The continuous-optimization procedure uses the analytic outer-loss
derivative only when all feasibility, stationarity, multiplier-sign,
complementarity, rank, conditioning, and support-interiority checks pass. At
active-set transitions, probability-floor contacts, or failed checks, it
switches to bounded finite differences, using one-sided differences at the
boundary of the outer domain. Sequential least-squares programming (SLSQP)
solves the inner convex program, and a multistart limited-memory
Broyden--Fletcher--Goldfarb--Shanno algorithm with box constraints (L-BFGS-B)
performs the continuous outer optimization. Appendix~\ref{app:solver} gives
the implementation details. The solution from the discrete grid search is
retained as a hard incumbent, so the continuous procedure cannot return a
worse fit, up to the stated numerical tolerances.

  % \vscomment{Can you de-AI the paragraph below? None of the quantities like $A_S$ or $D_{m,S}$ are defined, and dimensions for most matrices is not defined. It would be useful to first write down $K_\gamma$ in form of $Ax\leq b$ in the main text so that these matrices can be defined properly. Note that $C_S$ is different here than in the Appendix. There are also many acronyms that have no explanation. It'd be good to mention explicitly that derivations are in Appendix XYZ.}

  

% \begin{definition}[Slack parameterizations]
% \label{def:slack-params}
% We consider three nested parameterizations of $\gamma\in\Real_+^{\sum_k|A_k|}$:
% \begin{itemize}[leftmargin=*, itemsep=2pt, topsep=2pt]
% \item \emph{scalar} (1 parameter): $\gamma_{k,a}=\epsilon$ for all $(k,a)$;
% \item \emph{per-player} ($N$ parameters): $\gamma_{k,a}=\epsilon_k$ for all $a\in A_k$;
% \item \emph{per-action} ($\sum_k|A_k|$ parameters): the full vector $\gamma_{k,a}$, one slack per (player, action) pair.
% \end{itemize}
% We refer to the per-action parameterization throughout as \emph{CQRE-pa}.
% \end{definition}




\paragraph{Comparison between CQRE and Logit-QRE}
CQRE-pa differs from Logit-QRE in two ways: it ranges over joint distributions in the obedience polytope rather than products of marginals, and its slack vector is indexed by (player, action) pairs rather than by player alone. We examine each in turn.

\emph{(a) Correlation (joint vs.\ product).}
Logit-QRE is by construction a product measure across players, $\rho=\sigma_1\otimes\sigma_2$
\citep{mckelvey1995qre}, whereas \emph{every} CQRE---including the scalar one---ranges
over joint distributions in the obedience polytope. Let $\hat p_k$ denote the marginal of $\hat p$ on player $k$'s actions, and let $\hat p_1\otimes\cdots\otimes\hat p_N$ denote the product of those marginals. Writing $\log(\hat p/q) = \log\bigl(\hat p / (\hat p_1\otimes\cdots\otimes\hat p_N)\bigr) + \sum_k \log(\hat p_k/q_k)$ and taking expectation under $\hat p$ gives, for any product distribution $q = q_1\otimes\cdots\otimes q_N$,
\begin{align*}
\KL(\hat p \,\|\, q) &\;=\; I(\hat p) \;+\; \sum_k \KL(\hat p_k \,\|\, q_k),
\\
I(\hat p) &\;:=\; \KL\bigl(\hat p \,\big\|\, \hat p_1\otimes\cdots\otimes\hat p_N\bigr) \;=\; \sum_k H(\hat p_k) - H(\hat p) \;\ge\; 0,
\end{align*}
with equality iff $\hat p$ factorizes. The second sum on the right is minimized at $q_k = \hat p_k$, so every product-form predictor --- Logit-QRE included --- satisfies $\KL(\hat p \,\|\, p_{\text{Logit-QRE}}) \ge I(\hat p)$.
%\vscomment{\bfseries This needs more detail in the derivation---what is $\hat{\rho}_k$? Are you saying that you'll get the KL divergence between $\rho$ and the independent distribution obtained from the marginals? (This is true.)} 
When two LLMs read the same prompt and coordinate on a focal set of profiles---e.g.\ the diagonal of
a coordination game, where each plays $A$ exactly when the other does---$\hat p$ is
strongly correlated, $I(\hat p)\gg 0$, and Logit-QRE must pay this entire floor, while
CQRE places mass directly on the correlated cells and is not forced to incur this floor.  This is the
mechanism behind \emph{correlated} collapse.  It is \emph{absent} for single-cell
collapse onto a pure Nash profile, where $\hat p$ is essentially a product,
$I(\hat p)\approx 0$, and Logit-QRE is competitive---consistent with the two regimes in
which Logit-QRE wins (Section~\ref{sec:multigame}).






\emph{(b) Per-action slack (vector vs.\ scalar).}
Correlation alone does not separate the three CQRE parameterizations, since all of them
yield joint distributions; the per-action vector adds a second, orthogonal freedom.  In the
exponential form~\eqref{eq:gibbs} each multiplier $\lambda_{k,a_k,\widetilde a_k}$
scales a deviation payoff in the exponent.  A single $\beta$ per player is symmetric
across that player's own actions and cannot encode a label-specific preference independently of payoffs, whereas a
per-(player, action) $\gamma$ loosens the obedience constraint on one action only.
This is what represents \emph{action-label bias}---the systematic over-selection of a
particular label under relabeling---and lets a symmetric game support asymmetric
marginals.  The empirical gap between CQRE-pa and scalar/per-player CQRE indicates the value of this additional flexibility, since all three already share the correlation advantage of~(a).

Together, a \emph{joint distribution} can beat a product distribution for correlated play~(a), and a \emph{vector}
$\gamma$ beats a scalar on directional, per-label distortions~(b).  CQRE-pa is the
simplest notion in the set of alternatives we have considered that has both flexibilities, while remaining nested in the
maximum-entropy CE framework and inheriting its existence/uniqueness guarantees
(Theorem~\ref{thm:exists}).

\paragraph{Experimental setup.}
  For fixed $\gamma$, the inner program of Lemma~\ref{lem:inner-convex} is solved with SLSQP~\citep{kraft2005slsqp} under a probability floor $\rho_{ij} \ge 10^{-12}$; each inner
solve takes at most $1$\,ms for $n \le 5$. The discrete grid search fits the outer slack by coordinate-wise search over $\Gamma_0 = \{0,0.005,0.01,0.02,0.05,0.1,0.2\}$; the continuous
optimizer fits it with the guarded method above.  Appendix~\ref{app:solver} gives the algorithms. We compare CQRE-pa against five alternatives:
\emph{mixed Nash}, the product mixed-strategy profile closest to $\hat p$ in $\KL$; \emph{exact CQRE}, i.e.\ $\rho^\star_0$; the \emph{Logit-QRE-product}; and CQRE \emph{scalar}
and \emph{per-player} from Definition~\ref{def:slack-params}. For the all-12 robustness analysis we separately extend only the Logit precision domain to the compactified interval
$[0,\infty]$. For the
original weighted-RPS, multi-game, and three-player LLM experiments, we draw
  $B=1000$ multinomial bootstrap resamples and refit the compared notions.  The
  Selten--Chmura human table instead uses $B=2000$ subject-group resamples, and the all-12
  analyses use $B=2000$ synchronized dependence-aware or provider-time-block resamples as
  specified in Section~\ref{sec:selten-all12}; the relevant fitting parameters are refit
  within each replicate.  Where a paired interval is reported, it is formed from
  \[
  \Delta^{(b)} \;=\; \KL\big(\hat p^{(b)} \,\|\, p^{(b)}_{\textnormal{CQRE-pa}}\big) \;-\; \KL\big(\hat p^{(b)} \,\|\, p^{(b)}_{\textnormal{Logit-QRE}}\big);
  \]
  the pair is a \emph{CQRE-pa win} if this interval lies fully below zero, a \emph{Logit win} if fully above, and a \emph{tie} otherwise.

% =====================================================================


==> sections/04_empirical_evaluation.tex <==
\section{Empirical Evaluation}
\label{sec:empirical}
% =====================================================================

We evaluate how closely CQRE-pa fits empirical joint play in the Selten--Chmura human data; the weighted-RPS, multi-game, and three-player LLM corpora; and a sealed all-12 Selten extension whose reconstructed targets and estimands are stated explicitly. Throughout this section, CQRE-pa denotes the per-action specification fitted by
continuous slack optimization.  

\paragraph{Datasets / Corpora: }
\begin{itemize}[itemsep=1pt,topsep=2pt,leftmargin=*]
\item \textbf{Selten--Chmura human data} (Section~\ref{sec:selten}): 12 constant-sum
$2{\times}2$ games, with 12 independent subject groups in each of
\texttt{SC1}--\texttt{SC6}, 6 in each of \texttt{SC7}--\texttt{SC12}, and 800
realized action pairs per group.
\item \textbf{Weighted Rock-Paper-Scissors LLM round-robin} (Appendix~\ref{app:wrps-detail}): one
asymmetric weighted-RPS $3{\times}3$ game played by 6 frontier OpenAI deployments
(gpt-4o, gpt-4o-mini, gpt-4.1, gpt-4.1-mini,
gpt-5, gpt-5-mini); 20 completed pairs at $N{=}200$ matches each.
\item \textbf{Multi-game LLM tournament} (Section~\ref{sec:multigame}): the same 6
deployments across 7 normal-form games --- strongly-monotone $n\in\{3,5,7\}$
(\texttt{sm\_n3/5/7}) and rank-$r$ general-sum at $n{=}5$ (\texttt{rank1/2/3/4\_n5}) ---
yielding $7\times 21=147$ paired-bootstrap comparisons at $N{=}200$.
\item \textbf{Three-player extension} (Section~\ref{sec:three-player}): the same 6
deployments in all 216 ordered assignments for \texttt{jordan\_3p2a} and in the
56 model combinations with replacement for each of \texttt{shapley\_3p3a} and
\texttt{sm\_3p3a}, for 328 triplets total at $N{=}200$ matches per triplet.  The Jordan and Shapley
analyses are complete; the continuous \texttt{sm\_3p3a} bootstrap is left as a
placeholder.
\item \textbf{All-12 Selten extension} (Section~\ref{sec:selten-all12}):
a sealed 115,200-choice archive from the six AI models in all 12 presentations,
combined with published human frequencies.  The paired-seven same-target analysis
adds 86,400 new AI decisions used in the paired AAI construction
(201,600 accepted AI decisions in total) and fits
588 ordered targets separately; a distinct leave-one-strategic-family-out design
uses the sealed archive to test transfer across the six translation-equivalent game
families.
\end{itemize}

\subsection{Selten--Chmura human data}
\label{sec:selten}

CQRE-pa uses continuous slack optimization.  Both CQRE-pa and Logit-QRE are refitted in every bootstrap replicate.
Table~\ref{tab:selten} reports the point KL for each model and
the paired 95\% percentile interval for
$\Delta=\KL(\mathrm{CQRE\text{-}pa})-\KL(\mathrm{Logit\text{-}QRE})$ from
$B{=}2000$ synchronized hierarchical bootstrap replicates.  Each replicate
resamples whole subject groups and redraws 800 action pairs within each selected
group.  The target in each game is the equal-weight mean of its genuine
within-group joint distributions.  Four games favor
CQRE-pa, one favors Logit-QRE, and seven are unresolved.  Across all twelve
games, the equal-game point means are 0.0040 for CQRE-pa and 0.0093 for
Logit-QRE; the aggregate paired interval is strictly below zero.

 \begin{table}[H]
  \centering
  \caption{Fit to the twelve Selten--Chmura human-game
  targets. All six model
  columns report full-sample KL divergence. The last two columns
  compare continuous CQRE-pa with Logit-QRE: 
  $\Delta=\KL(\mathrm{CQRE\text{-}
  pa})-\KL(\mathrm{Logit\text{-}QRE})$.
  The interval is the paired 95\% percentile interval
  from $B{=}2000$. Green rows favor CQRE-pa, red
  rows favor Logit-QRE,
  and yellow rows are unresolved. }
\label{tab:selten}
  \scriptsize
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lrrrrrrrr}
  \toprule
  Game & Nash & Exact CQRE & Logit-QRE & CQRE sc. & CQRE
  pp. &
  CQRE-pa & $\Delta$ & Paired 95\% CI \\
  \midrule
  \rowcolor{cqrewin}SC1
  & 0.1910 & 0.1910 & 0.0183 & 0.0056 & 0.0019 &
  \textbf{0.0010} & $-0.0173$ & $[-0.0364,-0.0004]$ \\

  \rowcolor{tieyellow}SC2
  & 0.0947 & 0.0947 & 0.0053 & 0.0068 & 0.0051 &
  \textbf{0.0045} & $-0.0008$ & $[-0.0140,+0.0140]$ \\

  \rowcolor{logitwin}SC3
  & 0.0952 & 0.0952 & \textbf{0.0002} & 0.0356 & 0.0347
  &
  0.0261 & $+0.0258$ & $[+0.0124,+0.0385]$ \\

  \rowcolor{tieyellow}SC4
  & 0.0344 & 0.0344 & \textbf{0.0002} & 0.0147 & 0.0147
  &
  0.0093 & $+0.0091$ & $[-0.0012,+0.0183]$ \\

  \rowcolor{tieyellow}SC5
  & 0.0132 & 0.0132 & \textbf{0.0011} & 0.0062 & 0.0044
  &
  0.0032 & $+0.0021$ & $[-0.0074,+0.0089]$ \\

  \rowcolor{tieyellow}SC6
  & 0.0039 & 0.0039 & 0.0021 & 0.0017 & 0.0008 &
  \textbf{0.0005} & $-0.0016$ & $[-0.0053,+0.0019]$ \\

  \rowcolor{cqrewin}SC7
  & 0.4286 & 0.4286 & 0.0196 & 0.0035 & 0.0017 &
  \textbf{0.0008} & $-0.0188$ & $[-0.0328,-0.0077]$ \\

  \rowcolor{cqrewin}SC8
  & 0.0604 & 0.0604 & 0.0286 & 0.0008 & 0.0008 &
  \textbf{0.0007} & $-0.0279$ & $[-0.0516,-0.0083]$ \\

  \rowcolor{tieyellow}SC9
  & 0.0345 & 0.0345 & 0.0111 & 0.0028 & 0.0010 &
  \textbf{0.0004} & $-0.0108$ & $[-0.0322,+0.0234]$ \\

  \rowcolor{cqrewin}SC10
  & 0.0418 & 0.0418 & 0.0226 & 0.0045 & 0.0001 &
  \textbf{0.0000} & $-0.0226$ & $[-0.0369,-0.0019]$ \\

  \rowcolor{tieyellow}SC11
  & 0.0159 & 0.0159 & 0.0014 & 0.0035 & 0.0032 &
  \textbf{0.0013} & $-0.0001$ & $[-0.0090,+0.0070]$ \\

  \rowcolor{tieyellow}SC12
  & 0.0027 & 0.0027 & 0.0008 & 0.0008 & 0.0005 &
  \textbf{0.0003} & $-0.0005$ & $[-0.0041,+0.0014]$ \\
  \midrule
  \rowcolor{cqrewin}\textbf{All 12 games}
  & 0.0847 & 0.0847 & 0.0093 & 0.0072 & 0.0057 &
  \textbf{0.0040} & $\mathbf{-0.0053}$ &
  $\mathbf{[-0.0092,-0.0008]}$ \\
  \bottomrule
  \end{tabular}}
  \end{table}

  Within the CQRE family, the point estimates are consistent with the nesting order: continuous CQRE-pa has weakly lower KL than the grid-fitted per-player and scalar specifications in every game. Across all twelve games, equal-game mean KL falls from 0.0072 under scalar CQRE to 0.0057
  under per-player CQRE
  and 0.0040 under CQRE-pa. Relative to Logit-QRE, CQRE-
  pa has lower point KL
  in nine of the twelve games.  We next extend the same games with one-shot AI choices before returning to the LLM-only datasets.

\subsection{All-12 Selten extension: Human vs AI and AI vs AI}
\label{sec:selten-all12}

The 12 presentations form six payoff-translation-equivalent strategic
families, \texttt{SC1}/\texttt{SC7} through \texttt{SC6}/\texttt{SC12}.  Human
frequencies use periods 1--200.  The paired-seven analysis treats the six AI systems
and the human population as seven
agents and fits all $7\times7=49$ ordered row-agent--column-agent targets in every
presentation.  Its 588 targets comprise 432 AI--AI (AAI), 144 human--AI
(HAI) targets covering both orientations, and 12 human--human (HH) targets.  Each
AAI target uses 200 paired AI outcomes, and each HAI target uses a 200-decision
AI marginal.  The HH targets instead use the pooled released within-group human
distributions for periods 1--200.  Fresh AAI calls are paired by match ID;
reused archival responses are assigned to pairs without reference to their actions.
Each HAI target is the product of a pair-specific AI marginal and the corresponding
archival-human marginal, while HH preserves the observed within-group human joint.

Because HAI targets combine separately estimated human and AI marginals, they contain no information about within-match correlation between the two players’ actions.

For this same-target analysis, CQRE-pa is fitted by continuous optimization,
and both CQRE-pa and Logit-QRE are refitted in every one
of 2,000 synchronized paired bootstrap replicates.  We denote this continuous,
replicate-refitted protocol by $C$.  Both $C$ specifications use the same
continuous CQRE-pa estimator. The $C_{20}$ Logit-QRE specification means $\beta\in[0,20]$; $C_{\infty}$ is a separately labeled robustness specification that changes only that domain to the compactified $[0,\infty]$.  Here $\beta=\infty$ denotes the limiting mixed-Nash prediction, not a literal or precisely
measured degree of rationality.  Every target is fitted on itself.  Define $\Delta=\KL(\mathrm{CQRE\text{-}pa})-\KL(\mathrm{Logit\text{-}QRE})$, so negative
values favor CQRE-pa.

\begin{table}[H]

\centering
\caption{All-12 paired-seven same-target results.  Entries are full-sample
equal-target point means of $\Delta$, followed by synchronized 95\% percentile
intervals.  Targets are evaluation cells, not independent observational units;
HAI is constructed from marginal products, AAI combines are outcome-blind pairings, and HH uses observed within-group joints.
Row shading: green favors CQRE-pa and red favors Logit-QRE. }
\label{tab:selten-paired-seven-continuous}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrr}
\toprule
Population & Targets & $C_{20}$ & $C_{\infty}$ \\
\midrule
\rowcolor{cqrewin}ALL, target-weighted & 588 & $-0.00403\;[-0.00486,-0.00323]$ & $-0.00272\;[-0.00354,-0.00192]$ \\
\rowcolor{cqrewin}AAI & 432 & $-0.0088\;[-0.0098,-0.0078]$ & $-0.0073\;[-0.0082,-0.0063]$ \\
\rowcolor{logitwin}HAI, bidirectional & 144 & $+0.0105\;[+0.0090,+0.0118]$ & $+0.0112\;[+0.0098,+0.0124]$ \\
\rowcolor{cqrewin}HH & 12 & $-0.0053\;[-0.0092,-0.0008]$ & $-0.0053\;[-0.0092,-0.0008]$ \\
\bottomrule
\end{tabular}
}
\end{table}

The bidirectional HAI row averages the two ordered roles and should not be read as imposing or establishing role symmetry.

Removing the precision cap attenuates the target-weighted point
advantage by 32.4\% but does not change its sign: AAI and HH favor CQRE-pa, whereas
HAI favors Logit-QRE under both $C_{20}$ and $C_{\infty}$.  

At the full-sample point estimate, 475 of 588 Logit-QRE fits under $C_{\infty}$ remain
at $\beta\le20$, six select a finite $\beta>20$, and 107 select the limiting $\beta=\infty$ end point.  Extending the domain produces only minor numerical changes and leaves the qualitative conclusions unchanged.

\paragraph{Relative KL improvement.}
Table~\ref{tab:selten-paired-seven-levels} reports the KL levels behind the
paired differences in Table~\ref{tab:selten-paired-seven-continuous}.  The
percentage magnitude is
$100\lvert\KL_{\mathrm{Logit\text{-}QRE}}-\KL_{\mathrm{CQRE\text{-}pa}}\rvert
/\KL_{\mathrm{Logit\text{-}QRE}}$ and is labeled a reduction when CQRE-pa has
lower KL or an increase when it has higher KL.

\begin{table}[H]
\centering
\caption{Full-sample mean KL for continuous CQRE-pa and Logit-QRE under
$C_{20}$ and $C_{\infty}$.  Means are equally weighted over the targets in each
row.  The percentage is CQRE-pa's relative reduction or increase compared with
the corresponding Logit-QRE KL.  Green rows have lower CQRE-pa mean KL under
both domains; the red row has higher CQRE-pa mean KL under both.  These are
descriptive point estimates; bootstrap intervals are reported in
Table~\ref{tab:selten-paired-seven-continuous}.}
\label{tab:selten-paired-seven-levels}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
Population & Targets & CQRE-pa KL & Logit-QRE KL ($C_{20}$) & Change vs. $C_{20}$ & Logit-QRE KL ($C_{\infty}$) & Change vs. $C_{\infty}$ \\
\midrule
\rowcolor{cqrewin}ALL, target-weighted & 588 & \textbf{0.19744} & 0.20147 & \textbf{2.00\% reduction} & 0.20016 & \textbf{1.36\% reduction} \\
\rowcolor{cqrewin}AAI & 432 & \textbf{0.23526} & 0.24409 & \textbf{3.62\% reduction} & 0.24253 & \textbf{3.00\% reduction} \\
\rowcolor{logitwin}HAI, bidirectional & 144 & 0.10011 & \textbf{0.08963} & \textbf{11.69\% increase} & \textbf{0.08896} & \textbf{12.54\% increase} \\
\rowcolor{cqrewin}HH & 12 & \textbf{0.00400} & 0.00929 & \textbf{56.94\% reduction} & 0.00929 & \textbf{56.94\% reduction} \\
\bottomrule
\end{tabular}}
\end{table}

Across all 588 targets, continuous CQRE-pa lowers mean KL by 2.00\% relative
to $C_{20}$ Logit-QRE and by 1.36\% relative to $C_{\infty}$ Logit-QRE.  The
reduction is 3.62\% and 3.00\%, respectively, for AAI targets.  For HH play,
CQRE-pa lowers KL by 56.94\% under either Logit-QRE domain, from 0.00929 to
0.00400.  HAI is the exception: CQRE-pa has 11.69\% and 12.54\% higher mean KL.
A uniform-reference skill normalization gives the same qualitative comparison
and is reported in Appendix~\ref{app:selten-kl-skill}.

\paragraph{SC7 example.}
Figure~\ref{fig:sc7-all49-continuous} shows all 49 ordered SC7 targets.  The
aggregate favors CQRE-pa under both Logit-QRE precision domains: mean
$\Delta=-0.0906$ with 95\% interval $[-0.0949,-0.0848]$ under $C_{20}$, and
$\Delta=-0.0821$ with interval $[-0.0863,-0.0764]$ under $C_{\infty}$.

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/continuous/section5_contopt_sc7_all49_continuous.pdf}
\caption{SC7 comparison for all 49 ordered targets.  Each point plots Logit-QRE
KL on the horizontal axis against continuous CQRE-pa KL on the vertical axis;
points below the diagonal favor CQRE-pa.  Both models are refitted in every
bootstrap replicate.  The left panel uses $\beta\in[0,20]$, for which mean
$\Delta=-0.0906$ with 95\% interval $[-0.0949,-0.0848]$.  The right panel uses
$\beta\in[0,\infty]$, for which mean $\Delta=-0.0821$ with interval
$[-0.0863,-0.0764]$.  Horizontal and vertical bars are marginal bootstrap
intervals; marker outlines encode the paired-$\Delta$ verdict.  Arrows identify
the largest CQRE-pa improvement, the largest Logit-QRE improvement, and the HH
target.}
\label{fig:sc7-all49-continuous}
\end{figure}

\subsection{Multi-game LLM tournament: CQRE-pa versus Logit-QRE}
\label{sec:multigame}

Across 7 games and 21 model pairs each (147 paired comparisons),
Table~\ref{tab:multigame-verdicts} reports per-game paired-bootstrap outcomes.  CQRE-pa
wins $111/147 = 75.5\%$ of paired comparisons; the
$24$ Logit wins comprise 3 in \texttt{sm\_n3}, 16 in \texttt{rank2\_n5}, 3 in
\texttt{rank3\_n5}, and 2 in \texttt{rank4\_n5}; see
Section~\ref{sec:logit-wins}.
CQRE-pa uses continuous slack optimization.  The Logit-QRE comparison uses the stored raw-payoff, $\beta$ fits on $\beta\in[0,20]$. The corresponding seven-game results using $\beta\in[0,\infty]$ are reported in Appendix~\ref{app:multigame-logit-infinity}.

\begin{table}[H]
\centering
\caption{CQRE-pa against stored Logit-QRE fits with $\beta\in[0,20]$ on all 147 multi-LLM (game, pair) targets.  The KL columns report equal-target point means; bootstrap uses
($B{=}1000$) replicates. ``CQRE-pa wins'' means the 95\% CI of $\Delta=\KL_{\text{CQRE-pa}}-\KL_{\text{Logit-QRE}}$ is fully
below zero.  Green rows contain more CQRE-pa wins than Logit-QRE wins; the red row contains more Logit-QRE wins.}
\label{tab:multigame-verdicts}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\toprule
Game & $n$ & pairs & CQRE-pa KL & Stored Logit-QRE KL & CQRE-pa wins & Unresolved & Logit wins \\
\midrule
\rowcolor{cqrewin}\texttt{sm\_n3}     & 3 & 21 & 0.6157 & 10.613 & \textbf{18} & 0 & 3 \\
\rowcolor{cqrewin}\texttt{sm\_n5}     & 5 & 21 & 0.8648 & 1.0050 & \textbf{21} & 0 & 0 \\
\rowcolor{cqrewin}\texttt{sm\_n7}     & 7 & 21 & 1.2090 & 1.3872 & \textbf{21} & 0 & 0 \\
\rowcolor{cqrewin}\texttt{rank1\_n5}  & 5 & 21 & 1.2082 & 1.3948 & \textbf{21} & 0 & 0 \\
\rowcolor{logitwin}\texttt{rank2\_n5} & 5 & 21 & 1.3358 & 1.0898 & 1  & 4 & \textbf{16} \\
\rowcolor{cqrewin}\texttt{rank3\_n5}  & 5 & 21 & 1.2924 & 7.4076 & \textbf{18} & 0 & 3 \\
\rowcolor{cqrewin}\texttt{rank4\_n5}  & 5 & 21 & 1.0759 & 1.1351 & \textbf{11} & 8 & 2 \\
\midrule
\textbf{Total} & & \textbf{147} & \textbf{1.0859} & 3.4332 & \textbf{111} (75.5\%) & 12 (8.2\%) & 24 (16.3\%) \\
\bottomrule
\end{tabular}}
\end{table}

The point columns reproduce the stored losses, evaluated with the original
$10^{-15}$ probability floor.  The synchronized bootstrap instead rescores
both fixed predictions with the same $10^{-12}$ floor.

Figures~\ref{fig:scatter-sm} and~\ref{fig:scatter-rank} plot per-pair $\KL_{\text{Logit-QRE}}$
(horizontal) against $\KL_{\text{CQRE-pa}}$ (vertical) for each game; points below the $y{=}x$
diagonal are pairs where CQRE-pa fits the empirical joint better. 

\begin{figure}[H]
\centering
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_sm_n3_continuous.pdf}\caption{\texttt{sm\_n3}}\end{subfigure}\hfill
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_sm_n5_continuous.pdf}\caption{\texttt{sm\_n5}}\end{subfigure}\\[6pt]
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_sm_n7_continuous.pdf}\caption{\texttt{sm\_n7}}\end{subfigure}
\caption{Strongly-monotone comparison using continuous CQRE-pa and stored
Logit-QRE fits with $\beta\in[0,20]$:
per-pair $\KL_{\text{Logit-QRE}}$ vs.\ $\KL_{\text{CQRE-pa}}$ on each
of the 21 model pairs.  Error bars are marginal 95\% intervals from the same
synchronized fixed-prediction replay.  Points below $y{=}x$ favor CQRE-pa.  On \texttt{sm\_n5} and
\texttt{sm\_n7} every point is below the diagonal ($21/21$ sweep); on \texttt{sm\_n3},
$18/21$ are below and the 3 above are gpt-5-family self/near-self pairs collapsing onto the unique
pure Nash (Section~\ref{sec:logit-wins}).  Arrows identify the gpt-5-family
self/near-self outliers discussed below.}
\label{fig:scatter-sm}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_rank1_n5_continuous.pdf}\caption{\texttt{rank1\_n5}}\end{subfigure}\hfill
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_rank2_n5_continuous.pdf}\caption{\texttt{rank2\_n5}}\end{subfigure}\\[6pt]
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_rank3_n5_continuous.pdf}\caption{\texttt{rank3\_n5}}\end{subfigure}\hfill
\begin{subfigure}{0.48\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_rank4_n5_continuous.pdf}\caption{\texttt{rank4\_n5}}\end{subfigure}
\caption{Rank-$r$ general-sum comparison using continuous CQRE-pa and stored
Logit-QRE fits with $\beta\in[0,20]$,
$n{=}5$: per-pair $\KL_{\text{Logit-QRE}}$ vs.\
$\KL_{\text{CQRE-pa}}$.  Error bars are marginal 95\% intervals from the same
synchronized fixed-prediction replay.  CQRE-pa sweeps $r{=}1$ ($21/21$).
\texttt{rank2\_n5} is the largest inversion
($16$ Logit wins, $4$ unresolved, and $1$ CQRE-pa win); \texttt{rank3\_n5} and
\texttt{rank4\_n5} contain $3$ and $2$ additional Logit wins, respectively.
Arrows identify the gpt-5-family self/near-self outliers.}
\label{fig:scatter-rank}
\end{figure}

\paragraph{Where Logit wins.}
\label{sec:logit-wins}
The 24 strict Logit-QRE wins span four games.  Sixteen occur in
\texttt{rank2\_n5}, making that game the clearest concentration of Logit wins.
The label refers to the rank-two component $M=UV^\top$ in the construction
$R_1=K+M$ and $R_2=K-M$; the realized payoff matrices themselves have full rank,
and this association does not identify a causal mechanism.  Three further wins
occur for the gpt-5-family targets in \texttt{sm\_n3}.  Their empirical joints
place 98--99\% on $(A,A)$, the game's unique pure Nash.  The fitted Logit-QRE
distribution is correspondingly nearly degenerate at $(A,A)$, whereas the fitted
maximum-entropy CQRE-pa distributions remain diffuse.  The remaining five
wins---three in \texttt{rank3\_n5} and two in \texttt{rank4\_n5}---are
target-specific.  Table~\ref{tab:sm-anomaly} records the contrasting outcomes
in \texttt{sm\_n5} and \texttt{sm\_n7}; these comparisons are descriptive and
do not by themselves establish a mechanism.

\paragraph{Gpt-5-family targets account for much of the heterogeneity.}
\label{sec:gpt5-family}
Stratifying the $147$ paired comparisons by gpt-5-family membership ($21$ self/near-self
pairs) versus the other $126$ reveals a $\sim\!3$-nat separation in the mean paired
$\Delta = \KL_{\text{CQRE-pa}} - \KL_{\text{Logit-QRE}}$: $+0.25$ on gpt-5 pairs
versus $-2.78$ on the rest.  The gpt-5-family targets also show more
concentrated empirical play in every game; separately, their mean
$\KL_{\text{CQRE-pa}}$ is $1.7$--$3.3\times$ the within-game mean for the
remaining targets.  These are descriptive associations, and the sign of the
comparison varies with game structure.  \emph{(i)}~In \texttt{sm\_n3}, whose
concentration cell is a pure Nash with mirror-symmetric marginals, the
gpt-5-family mean is $\Delta=+1.43$.  In \texttt{rank2\_n5}, whose construction
contains the rank-two component $M=UV^\top$, the corresponding mean is
$\Delta=+1.14$.  Logit-QRE wins $3/3$ gpt-5-family comparisons in each game,
but these associations do not isolate the mechanism.  \emph{(ii)}~On
\texttt{sm\_n5}, \texttt{sm\_n7},
\texttt{rank1\_n5}, and \texttt{rank4\_n5}, CQRE-pa wins all 12 gpt-5-family
comparisons; the four game-level gpt-5-family mean
deltas range from $-0.67$ to $-0.18$.  The three gpt-5-family pairs in
\texttt{rank3\_n5} favor Logit-QRE, but we do not attribute those cases to either
structural pattern above.

\paragraph{Self-play vs cross-play}
\label{sec:self-vs-cross}
The color split in Figures~\ref{fig:scatter-sm}--\ref{fig:scatter-rank} between
self-play ($42$ pairs) and cross-play ($105$ pairs) is descriptive rather than
explanatory.  Pooled across the $147$ pairs, mean $\Delta$ is $-2.22$ on self-play
and $-2.40$ on cross-play; the CQRE-pa/Logit-QRE/unresolved shares are
$74\%/19\%/7\%$ for self-play and $76\%/15\%/9\%$ for cross-play. We do not
report a paired interval or test for this pooled contrast, so these summaries
alone do not establish whether self-play and cross-play differ. We retain the
color distinction in the scatters only as a visual locator.

\begin{table}[H]
\centering
\caption{Pure-Nash and marginal-symmetry conditions across the strongly-monotone family.
The reported $\Delta$ values compare continuous CQRE-pa with stored Logit-QRE fits under
$\beta\in[0,20]$.  Each synchronized
fixed-prediction interval excludes zero in the direction indicated by the row
color.}
\label{tab:sm-anomaly}
\small
\begin{tabular}{lcccccc}
\toprule
Game & $n$ & Pure Nash & Collapse cell & Cell is Nash? & Sym.\ marginals? & gpt-5 self verdict \\
\midrule
\rowcolor{logitwin}\texttt{sm\_n3} & 3 & $\{(A,A)\}$ & $(A,A)$ & \textbf{Yes} & \textbf{Yes} & Logit-QRE ($\Delta{=}{+}1.47$) \\
\rowcolor{cqrewin}\texttt{sm\_n5}  & 5 & None & $(B,B)$ & No & No & CQRE-pa ($\Delta{=}{-}0.46$) \\
\rowcolor{cqrewin}\texttt{sm\_n7}  & 7 & $\{(B,B)\}$ & $(B,B)$ & Yes & No & CQRE-pa ($\Delta{=}{-}0.80$) \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Effective dimensionality of the continuously fitted slacks.}
In a separate eight-game size sweep over $n=3,\ldots,10$, we take the
componentwise-minimal per-action slack vector associated with each of the 21
continuously optimized CQRE-pa fits.  Stacking these vectors and centering each
coordinate gives a $21\times 2n$ matrix.  Let $r_{90}$ be the smallest number of
singular directions accounting for at least 90\% of its squared singular-value
mass.  Across the eight games, $r_{90}$ is
$\{2,4,3,4,6,7,4,7\}$, or 22--50\% of the nominal dimension.  This is a
descriptive compression diagnostic; it does not identify a behavioral latent
dimension or by itself rule out overfitting.  Appendix~\ref{app:supplementary-empirical}
reports the full rank table and its pair-resampling ranges.

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/continuous/continuous_gamma_scree_2x4.pdf}
\caption{Singular-value spectra of the centered componentwise-minimal slack
vectors from the continuous CQRE-pa fits.  Each panel contains the 21 model-pair
targets for one strongly-monotone game.  Bars show per-component variance
fractions, the red curve shows cumulative variance, the dashed horizontal line
marks 90\%, and the green line marks $r_{90}$.  The display is a descriptive
parameter-compression diagnostic.}
\label{fig:continuous-gamma-scree}
\end{figure}



\subsection{Three-player LLM play}
\label{sec:three-player}

The CQRE-pa specification extends to $N$-player games via the tensor form of \eqref{eq:cqre}.
We consider three 3-player games: \texttt{jordan\_3p2a}~\citep{jordan1993three}
(unique mixed Nash at uniform), \texttt{shapley\_3p3a}~\citep{shapley1964some}
(a 3-action best-response cycle with three pure Nash profiles), and \texttt{sm\_3p3a}
(3-player 3-action strongly-monotone-style, unique pure Nash at $(A,C,C)$).

\begin{table}[H]
\centering
\caption{Paired-refit comparison of continuous CQRE-pa and Logit-QRE with
$\beta\in[0,20]$.
Every Jordan and Shapley triplet is an exact tie under $B{=}1000$; the entries
in brackets are aggregate paired 95\% intervals.  The verified
\texttt{sm\_3p3a} point fit is shown, but its full $B{=}1000$ bootstrap remains
to be completed.}
\label{tab:three-player}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrr}
\toprule
Game & Structure & Triplets & CQRE-pa KL & Logit-QRE KL & $\Delta$ [95\% CI] \\
\midrule
\rowcolor{tieyellow}\texttt{jordan\_3p2a} & Cyclic, unique uniform Nash & 216 & 0.2562 & 0.2562 & $0\;[0,0]$ \\
\rowcolor{tieyellow}\texttt{shapley\_3p3a} & Best-response cycle, three pure Nash & 56 & 0.1850 & 0.1850 & $0\;[0,0]$ \\
\rowcolor{gray!15}\texttt{sm\_3p3a} & Strongly-monotone-style, unique $(A,C,C)$ Nash & 56 & 0.4950 & 0.6316 & \textit{Bootstrap pending} \\
\midrule
\textbf{Total} & & 328 & \multicolumn{3}{c}{\textit{To be completed}} \\
\bottomrule
\end{tabular}}
\end{table}

Figure~\ref{fig:scatter-3p} plots the completed Jordan and Shapley comparisons
from the paired-refit results and leaves the \texttt{sm\_3p3a} panel as
a placeholder.

\begin{figure}[H]
\centering
\begin{subfigure}{0.49\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_jordan_3p2a_continuous.pdf}\caption{\texttt{jordan\_3p2a} (216 triplets)}\end{subfigure}\hfill
\begin{subfigure}{0.49\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/scatter_shapley_3p3a_continuous.pdf}\caption{\texttt{shapley\_3p3a} (56 triplets)}\end{subfigure}\\[6pt]
\begin{subfigure}{0.49\textwidth}\centering\includegraphics[width=\linewidth]{figures/continuous/pendinginging.pdf}\caption{\texttt{sm\_3p3a} (56 triplets)}\end{subfigure}
\caption{Three-player scatter: $\KL_{\text{Logit-QRE}}$ vs.\ continuous
$\KL_{\text{CQRE-pa}}$.  On \texttt{jordan\_3p2a} and
\texttt{shapley\_3p3a}, both notions return the same fitted distribution for
every target, so every triplet lies on the diagonal.  The
full $B{=}1000$ \texttt{sm\_3p3a} bootstrap panel will be added after validation.}
\label{fig:scatter-3p}
\end{figure}

For Jordan and Shapley, continuous CQRE-pa and Logit-QRE coincide on every
target.  On \texttt{sm\_3p3a}, CQRE-pa has the lower point KL for all 56
triplets.  Its point fit is verified, but we do not report an inferential
verdict until the full $B{=}1000$ bootstrap is complete.

\paragraph{Reproducibility}
\label{sec:reproducibility-main}

We rerun the full numerical pipeline on every saved transcript under a locked Python
environment.  The completed continuous CQRE-pa fits and bootstrap outputs used in
this section pass their stored validation checks.  Full audit specification and
per-target diagnostics are in Appendix~\ref{app:reproducibility}.
The sealed all-12 pipeline additionally verifies every one of 2,352
target-level summaries (588 targets under four prespecified analysis lanes),
all 156 extended aggregate summaries, and the audits of continuous optimization
and dependence-aware resampling.













% \paragraph{Replication under other distance metrics.}
% \sout{The dominance is not specific to KL divergence.  Appendix~\ref{app:extra-metrics} replicates the
% analysis using total variation, $L_2$ distance, and Rényi-$1/2$ divergence: CQRE-pa
% remains the best notion on the cross-game mean for every metric on the multigame corpus
% (Table~\ref{tab:extra-metrics-family}) and on $5$--$6$ of $7$ games per metric. }

% \vscomment{Do highlight that some of these are true metrics (so equivalent due to finite dimensional setting), but others like KL and Renyi are only divergences.}




==> sections/05_discussion_and_conclusion.tex <==
\section{Conclusion}
\label{sec:discussion}
% =====================================================================


 The human evidence comes first: observed Selten--Chmura within-group play
  is the most direct behavioral target, but it is a fixed and limited data set.  The
  all-12 extension broadens coverage with one-shot AI decisions while explicitly treating
  HAI and canonical AAI as reconstructed products rather than observed interactions.  In
  the 588-target same-target M$\infty$ comparison, the target-weighted mean favors CQRE-pa,
  as do the AAI and HH aggregates, while HAI favors Logit-QRE.  The apparently different
  held-out-family result answers another question: CQRE-pa improves on the published
  raw-payoff one-$\beta$ comparator for pooled HAI and canonical AAI, but a
  player-normalized two-$\beta$ robustness comparator reverses those pooled conclusions.
  Neither result licenses a claim that CQRE-pa always wins.

  Algorithmically, the continuous outer-$\gamma$ estimator replaces an
  arbitrary grid endpoint with a complete bounded domain, differentiates the inner
  maximum-entropy solution through a guarded KKT system, and retains the grid incumbent.
  It improves many fixed-target fits and substantially reduces complete inner solves, but
  remains a multi-start local search rather than a global certificate.  Canonicalization
  is required before interpreting slack geometry because inactive coordinates are not
  identified.  The resulting low-dimensional patterns are descriptive and are compatible
  with the product-geometry calibration.

  The claim throughout is descriptive: which static joint-distribution benchmark best
  describes existing strategic play. Targetwise win counts, aggregate KL
  magnitudes, same-target fitting, and held-out-family prediction are complementary but
  non-interchangeable summaries.  The ex-post HAI oracle benchmark places 71.1\% of AI
  mass on payoff-maximizing actions and finds mean normalized regret of 2.49\%, but it is
  not evidence that the one-shot models observed or learned the human distribution.  On a
  uniform-joint reference scale, continuous CQRE-pa and extended-domain Logit remove
  64.51\% and 64.02\%, respectively, of aggregate target KL; the remaining difference is
  $0.00393$ bits per choice.  Utility regret and predictive KL answer different questions
  and are reported separately.

==> tables/ci/rank1_n5_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{rank1\_n5}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_rank1_n5}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4.1 vs gpt-4o-mini & 3.42[2.61,4.29] & 0.92[0.80,1.05] & 1.46[1.32,1.61] & 0.92[0.80,1.05] & 0.87[0.75,0.99] & \textbf{0.84[0.74,0.95]} \\
gpt-4.1 vs gpt-4o & 2.39[1.85,3.00] & 0.99[0.87,1.10] & 1.55[1.40,1.70] & 0.99[0.87,1.10] & 0.91[0.78,1.02] & \textbf{0.87[0.76,0.97]} \\
gpt-4o-mini vs gpt-5 & 3.69[2.75,4.71] & 1.06[0.93,1.20] & 1.11[0.98,1.25] & 1.01[0.88,1.15] & 0.97[0.84,1.10] & \textbf{0.89[0.76,1.02]} \\
gpt-4o vs gpt-5-mini & 2.02[1.51,2.64] & 1.16[1.05,1.28] & 1.50[1.35,1.64] & 1.16[1.05,1.28] & 1.05[0.93,1.18] & \textbf{0.97[0.86,1.09]} \\
gpt-4o-mini vs gpt-5-mini & 2.32[1.71,3.01] & 1.15[1.03,1.27] & 1.36[1.22,1.50] & 1.14[1.02,1.26] & 1.05[0.92,1.17] & \textbf{0.97[0.85,1.09]} \\
gpt-4o vs gpt-4o-mini & 3.83[2.99,4.79] & 1.06[0.90,1.21] & 1.77[1.61,1.93] & 1.06[0.90,1.21] & 1.05[0.89,1.20] & \textbf{0.99[0.85,1.13]} \\
gpt-4.1-mini vs gpt-4o-mini & 3.89[3.09,4.76] & 1.11[0.99,1.24] & 1.90[1.70,2.10] & 1.11[0.99,1.24] & 1.04[0.92,1.16] & \textbf{1.02[0.91,1.14]} \\
gpt-4o vs gpt-4o & 3.49[2.77,4.35] & 1.11[0.96,1.25] & 1.99[1.81,2.16] & 1.11[0.96,1.25] & 1.10[0.96,1.24] & \textbf{1.04[0.90,1.17]} \\
gpt-4.1 vs gpt-4.1 & 1.89[1.57,2.32] & 1.20[1.09,1.31] & 1.75[1.63,1.89] & 1.20[1.09,1.31] & 1.13[1.03,1.24] & \textbf{1.08[0.98,1.17]} \\
gpt-4o-mini vs gpt-4o-mini & 6.74[5.44,8.11] & 1.21[1.06,1.37] & 1.73[1.58,1.89] & 1.21[1.06,1.37] & 1.16[1.02,1.32] & \textbf{1.09[0.96,1.23]} \\
gpt-4.1-mini vs gpt-4o & 3.13[2.55,3.77] & 1.21[1.07,1.36] & 2.04[1.83,2.25] & 1.21[1.07,1.36] & 1.14[1.00,1.28] & \textbf{1.10[0.97,1.24]} \\
gpt-4o vs gpt-5 & 1.79[1.41,2.30] & 1.32[1.20,1.45] & 1.58[1.44,1.75] & 1.31[1.19,1.44] & 1.21[1.09,1.35] & \textbf{1.12[1.00,1.25]} \\
gpt-4.1 vs gpt-5 & 1.87[1.43,2.38] & 1.45[1.33,1.58] & 1.61[1.47,1.76] & 1.43[1.31,1.56] & 1.33[1.20,1.45] & \textbf{1.20[1.07,1.32]} \\
gpt-4.1 vs gpt-4.1-mini & 2.11[1.89,2.42] & 1.39[1.28,1.50] & 2.03[1.89,2.18] & 1.39[1.28,1.50] & 1.30[1.19,1.40] & \textbf{1.24[1.14,1.35]} \\
gpt-4.1-mini vs gpt-5 & 2.20[1.84,2.65] & 1.55[1.43,1.70] & 1.85[1.70,2.02] & 1.53[1.41,1.67] & 1.41[1.30,1.55] & \textbf{1.29[1.17,1.43]} \\
gpt-4.1 vs gpt-5-mini & \textbf{1.34[1.26,1.44]} & 1.63[1.51,1.76] & 1.82[1.71,1.94] & 1.62[1.50,1.74] & 1.53[1.41,1.65] & 1.43[1.31,1.55] \\
gpt-4.1-mini vs gpt-5-mini & 2.25[1.93,2.66] & 1.80[1.68,1.91] & 2.02[1.89,2.15] & 1.78[1.66,1.89] & 1.65[1.54,1.76] & \textbf{1.53[1.42,1.63]} \\
gpt-5 vs gpt-5 & 2.18[1.65,2.84] & 1.97[1.81,2.13] & 1.75[1.57,1.94] & 1.75[1.57,1.94] & 1.75[1.57,1.94] & \textbf{1.57[1.41,1.74]} \\
gpt-4.1-mini vs gpt-4.1-mini & 3.14[2.82,3.52] & 1.96[1.79,2.14] & 2.79[2.59,2.99] & 1.96[1.79,2.14] & 1.89[1.72,2.07] & \textbf{1.81[1.65,1.98]} \\
gpt-5 vs gpt-5-mini & \textbf{1.67[1.47,1.95]} & 2.18[2.03,2.33] & 2.07[1.91,2.23] & 2.07[1.91,2.23] & 2.03[1.88,2.19] & 1.85[1.70,2.00] \\
gpt-5-mini vs gpt-5-mini & \textbf{1.75[1.65,1.84]} & 2.53[2.39,2.67] & 2.48[2.35,2.62] & 2.48[2.35,2.62] & 2.40[2.26,2.55] & 2.19[2.06,2.32] \\
\end{longtable}}


==> tables/ci/rank2_n5_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{rank2\_n5}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_rank2_n5}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4.1 vs gpt-4o & 11.36[9.81,13.04] & \textbf{0.72[0.61,0.83]} & 1.08[0.94,1.23] & 0.88[0.76,1.00] & 0.85[0.74,0.99] & 0.78[0.66,0.90] \\
gpt-4.1 vs gpt-4o-mini & 7.33[5.81,8.91] & \textbf{0.80[0.68,0.93]} & 1.04[0.90,1.18] & 0.92[0.80,1.06] & 0.87[0.74,1.01] & 0.80[0.68,0.93] \\
gpt-4o vs gpt-4o & 7.83[6.35,9.41] & 0.84[0.72,0.96] & 1.07[0.94,1.20] & 0.96[0.84,1.09] & 0.94[0.82,1.06] & \textbf{0.83[0.72,0.95]} \\
gpt-4.1-mini vs gpt-4o & 11.56[9.80,13.24] & \textbf{0.78[0.66,0.91]} & 1.21[1.05,1.38] & 0.95[0.82,1.10] & 0.93[0.80,1.08] & 0.85[0.73,0.99] \\
gpt-4o vs gpt-4o-mini & 6.77[5.38,8.09] & 1.06[0.89,1.24] & 1.18[1.02,1.36] & 1.15[0.97,1.33] & 1.14[0.97,1.32] & \textbf{1.04[0.87,1.21]} \\
gpt-4o vs gpt-5 & 16.20[14.34,17.97] & \textbf{0.90[0.79,1.02]} & 1.55[1.38,1.71] & 1.11[0.99,1.25] & 1.09[0.97,1.23] & 1.06[0.94,1.19] \\
gpt-4.1 vs gpt-4.1 & 14.49[12.80,16.19] & \textbf{0.95[0.83,1.08]} & 1.38[1.22,1.54] & 1.17[1.04,1.30] & 1.16[1.03,1.30] & 1.06[0.93,1.20] \\
gpt-4o-mini vs gpt-4o-mini & 4.13[3.10,5.27] & 1.12[0.96,1.29] & 1.18[1.03,1.34] & 1.18[1.03,1.34] & 1.17[1.02,1.34] & \textbf{1.06[0.91,1.23]} \\
gpt-4.1-mini vs gpt-4o-mini & 7.77[6.18,9.33] & 1.08[0.96,1.19] & 1.37[1.26,1.48] & 1.21[1.09,1.32] & 1.18[1.06,1.29] & \textbf{1.07[0.96,1.17]} \\
gpt-4.1 vs gpt-4.1-mini & 14.84[13.09,16.54] & \textbf{1.13[0.98,1.27]} & 1.64[1.46,1.82] & 1.34[1.19,1.50] & 1.34[1.19,1.50] & 1.25[1.10,1.41] \\
gpt-4o vs gpt-5-mini & 17.98[16.34,19.54] & \textbf{1.13[1.03,1.25]} & 1.83[1.70,1.98] & 1.36[1.24,1.49] & 1.34[1.22,1.47] & 1.31[1.20,1.45] \\
gpt-4.1 vs gpt-5 & 18.27[16.56,19.81] & \textbf{1.08[0.93,1.23]} & 1.65[1.50,1.82] & 1.35[1.22,1.48] & 1.32[1.19,1.45] & 1.31[1.18,1.45] \\
gpt-4o-mini vs gpt-5 & 16.47[14.69,18.21] & \textbf{1.16[1.04,1.29]} & 1.87[1.70,2.05] & 1.38[1.24,1.53] & 1.36[1.22,1.51] & 1.33[1.19,1.48] \\
gpt-4.1-mini vs gpt-4.1-mini & 11.09[9.34,12.73] & \textbf{1.27[1.16,1.39]} & 1.76[1.62,1.91] & 1.48[1.36,1.61] & 1.44[1.32,1.57] & 1.33[1.21,1.46] \\
gpt-4o-mini vs gpt-5-mini & 15.36[13.57,17.17] & \textbf{1.26[1.14,1.39]} & 2.01[1.85,2.19] & 1.45[1.33,1.59] & 1.43[1.30,1.56] & 1.39[1.27,1.53] \\
gpt-4.1 vs gpt-5-mini & 19.22[17.53,20.86] & \textbf{1.38[1.23,1.53]} & 1.89[1.74,2.04] & 1.54[1.43,1.67] & 1.53[1.41,1.65] & 1.51[1.40,1.64] \\
gpt-4.1-mini vs gpt-5-mini & 18.10[16.43,19.73] & \textbf{1.35[1.23,1.47]} & 2.05[1.90,2.21] & 1.61[1.47,1.75] & 1.58[1.44,1.73] & 1.55[1.42,1.69] \\
gpt-4.1-mini vs gpt-5 & 19.48[17.88,21.15] & \textbf{1.39[1.26,1.53]} & 2.08[1.91,2.26] & 1.66[1.52,1.80] & 1.63[1.49,1.78] & 1.62[1.48,1.77] \\
gpt-5 vs gpt-5 & 26.41[25.67,27.03] & \textbf{1.25[1.14,1.36]} & 2.82[2.68,2.96] & 2.61[2.48,2.74] & 2.59[2.46,2.73] & 2.54[2.42,2.67] \\
gpt-5 vs gpt-5-mini & 26.90[26.43,27.25] & \textbf{1.28[1.18,1.39]} & 2.88[2.76,3.02] & 2.63[2.50,2.76] & 2.62[2.49,2.76] & 2.54[2.42,2.67] \\
gpt-5-mini vs gpt-5-mini & 27.04[26.69,27.25] & \textbf{1.66[1.61,1.70]} & 2.97[2.89,3.04] & 2.65[2.55,2.74] & 2.64[2.55,2.73] & 2.61[2.52,2.69] \\
\end{longtable}}


==> tables/ci/rank3_n5_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{rank3\_n5}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_rank3_n5}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4o vs gpt-4o & 20.36[18.97,21.65] & 10.82[9.78,11.97] & 2.65[2.44,2.89] & 0.88[0.76,1.00] & 0.88[0.76,1.00] & \textbf{0.85[0.74,0.97]} \\
gpt-4o vs gpt-4o-mini & 22.14[20.88,23.31] & 11.42[10.43,12.46] & 2.92[2.68,3.17] & 0.99[0.87,1.12] & 0.99[0.87,1.11] & \textbf{0.96[0.85,1.09]} \\
gpt-4o vs gpt-5 & 12.74[10.96,14.44] & 5.11[4.21,5.98] & 2.00[1.73,2.29] & 1.13[1.03,1.25] & 1.09[0.99,1.21] & \textbf{0.97[0.86,1.09]} \\
gpt-4o-mini vs gpt-5 & 14.96[13.08,16.76] & 6.10[5.09,7.14] & 2.01[1.75,2.26] & 1.18[1.08,1.28] & 1.10[1.01,1.20] & \textbf{0.99[0.90,1.10]} \\
gpt-4o-mini vs gpt-5-mini & 14.24[12.42,15.90] & 6.08[5.15,6.98] & 2.12[1.85,2.41] & 1.10[1.00,1.21] & 1.07[0.97,1.17] & \textbf{1.00[0.90,1.11]} \\
gpt-4o vs gpt-5-mini & 12.97[11.34,14.63] & 5.28[4.44,6.18] & 2.08[1.83,2.36] & 1.10[1.00,1.21] & 1.10[1.00,1.21] & \textbf{1.02[0.92,1.13]} \\
gpt-4.1 vs gpt-4o-mini & 22.08[20.70,23.34] & 10.66[9.69,11.66] & 3.29[3.08,3.51] & 1.10[0.99,1.22] & 1.10[0.99,1.22] & \textbf{1.06[0.95,1.18]} \\
gpt-4.1-mini vs gpt-4o-mini & 20.98[19.50,22.29] & 10.60[9.68,11.64] & 3.25[3.01,3.49] & 1.12[0.99,1.25] & 1.12[0.99,1.25] & \textbf{1.09[0.97,1.22]} \\
gpt-4o-mini vs gpt-4o-mini & 24.11[23.16,24.92] & 13.03[12.04,14.05] & 3.05[2.83,3.30] & 1.19[1.05,1.35] & 1.18[1.03,1.33] & \textbf{1.15[1.01,1.31]} \\
gpt-4.1-mini vs gpt-4o & 20.43[18.99,21.89] & 9.74[8.71,10.77] & 3.24[2.96,3.52] & 1.21[1.06,1.36] & 1.21[1.06,1.36] & \textbf{1.16[1.01,1.31]} \\
gpt-4.1 vs gpt-5-mini & 15.29[13.65,17.06] & 4.87[4.15,5.60] & 2.58[2.27,2.88] & 1.35[1.23,1.48] & 1.33[1.22,1.45] & \textbf{1.19[1.07,1.32]} \\
gpt-4.1 vs gpt-4o & 21.08[19.69,22.39] & 10.57[9.49,11.58] & 3.27[3.01,3.51] & 1.22[1.07,1.36] & 1.22[1.07,1.36] & \textbf{1.20[1.05,1.33]} \\
gpt-4.1-mini vs gpt-5-mini & 13.92[12.21,15.76] & 5.03[4.27,5.82] & 2.63[2.34,2.93] & 1.44[1.31,1.57] & 1.42[1.31,1.54] & \textbf{1.27[1.16,1.38]} \\
gpt-4.1 vs gpt-5 & 15.33[13.66,17.15] & 5.10[4.33,5.89] & 2.73[2.42,3.05] & 1.58[1.45,1.70] & 1.52[1.39,1.64] & \textbf{1.32[1.19,1.43]} \\
gpt-4.1-mini vs gpt-5 & 14.43[12.61,16.15] & 5.33[4.50,6.19] & 2.92[2.61,3.26] & 1.67[1.54,1.80] & 1.61[1.48,1.74] & \textbf{1.41[1.29,1.54]} \\
gpt-4.1-mini vs gpt-4.1-mini & 23.43[22.22,24.45] & 9.88[9.09,10.67] & 4.13[3.86,4.39] & 1.71[1.55,1.87] & 1.68[1.53,1.83] & \textbf{1.61[1.46,1.76]} \\
gpt-4.1 vs gpt-4.1 & 22.65[21.29,23.80] & 10.03[9.36,10.71] & 4.02[3.75,4.28] & 1.67[1.52,1.84] & 1.66[1.52,1.81] & \textbf{1.61[1.46,1.77]} \\
gpt-4.1 vs gpt-4.1-mini & 22.66[21.42,23.78] & 9.94[9.27,10.61] & 3.99[3.73,4.23] & 1.69[1.55,1.83] & 1.66[1.53,1.80] & \textbf{1.62[1.48,1.75]} \\
gpt-5-mini vs gpt-5-mini & 1.92[1.89,1.96] & \textbf{1.35[1.32,1.39]} & 2.21[2.21,2.23] & 2.21[2.21,2.23] & 2.20[2.18,2.23] & 2.04[1.99,2.11] \\
gpt-5 vs gpt-5-mini & 1.89[1.81,1.98] & \textbf{1.30[1.28,1.33]} & 2.16[2.09,2.22] & 2.16[2.09,2.22] & 2.16[2.09,2.22] & 2.05[1.96,2.15] \\
gpt-5 vs gpt-5 & 1.97[1.86,2.08] & \textbf{1.31[1.28,1.34]} & 2.18[2.09,2.27] & 2.18[2.09,2.27] & 2.18[2.09,2.27] & 2.18[2.09,2.26] \\
\end{longtable}}


==> tables/ci/rank4_n5_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{rank4\_n5}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_rank4_n5}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4.1 vs gpt-4o-mini & 10.12[8.65,11.85] & 0.75[0.65,0.86] & 1.36[1.17,1.55] & 0.82[0.71,0.93] & 0.80[0.69,0.92] & \textbf{0.72[0.63,0.83]} \\
gpt-4o vs gpt-4o-mini & 10.95[9.38,12.64] & 0.83[0.73,0.95] & 1.53[1.33,1.74] & 0.85[0.75,0.96] & 0.85[0.75,0.96] & \textbf{0.74[0.65,0.84]} \\
gpt-4o vs gpt-4o & 11.02[9.51,12.78] & 0.85[0.75,0.97] & 1.46[1.29,1.62] & 0.87[0.77,0.98] & 0.87[0.77,0.98] & \textbf{0.75[0.66,0.85]} \\
gpt-4.1 vs gpt-4o & 5.89[4.61,7.22] & 0.89[0.76,1.03] & 1.29[1.10,1.50] & 0.98[0.84,1.12] & 0.93[0.79,1.06] & \textbf{0.83[0.71,0.97]} \\
gpt-4o vs gpt-5 & 23.84[22.84,24.66] & 0.92[0.80,1.04] & 1.57[1.34,1.79] & 0.95[0.83,1.07] & 0.94[0.83,1.06] & \textbf{0.86[0.76,0.97]} \\
gpt-4.1-mini vs gpt-4o & 7.43[5.97,9.08] & \textbf{0.85[0.76,0.93]} & 1.45[1.29,1.63] & 0.96[0.85,1.06] & 0.91[0.81,1.01] & 0.88[0.78,0.97] \\
gpt-4.1-mini vs gpt-4o-mini & 8.61[7.06,10.11] & 0.91[0.82,1.02] & 1.85[1.66,2.05] & 0.97[0.87,1.07] & 0.96[0.86,1.06] & \textbf{0.88[0.79,0.98]} \\
gpt-4o vs gpt-5-mini & 22.47[21.27,23.64] & 0.94[0.84,1.05] & 1.79[1.58,2.01] & 1.01[0.92,1.11] & 0.98[0.88,1.08] & \textbf{0.89[0.81,0.99]} \\
gpt-4.1 vs gpt-4.1 & 5.79[4.54,7.13] & 0.98[0.86,1.11] & 1.47[1.31,1.65] & 1.19[1.06,1.34] & 1.05[0.93,1.19] & \textbf{0.97[0.85,1.09]} \\
gpt-4o-mini vs gpt-5 & 24.09[23.12,24.95] & 1.06[0.94,1.18] & 1.86[1.62,2.10] & 1.07[0.96,1.19] & 1.06[0.95,1.17] & \textbf{0.97[0.85,1.08]} \\
gpt-4.1 vs gpt-5 & 23.19[22.09,24.22] & \textbf{0.96[0.84,1.07]} & 1.53[1.36,1.73] & 1.11[0.98,1.23] & 1.06[0.94,1.18] & 0.98[0.87,1.09] \\
gpt-4o-mini vs gpt-4o-mini & 15.30[13.60,16.89] & 1.22[1.08,1.37] & 2.09[1.85,2.33] & 1.23[1.08,1.38] & 1.23[1.08,1.38] & \textbf{0.99[0.88,1.12]} \\
gpt-4o-mini vs gpt-5-mini & 23.72[22.73,24.64] & 1.07[0.95,1.20] & 2.01[1.77,2.27] & 1.11[1.00,1.23] & 1.10[0.99,1.22] & \textbf{1.00[0.89,1.13]} \\
gpt-4.1 vs gpt-5-mini & 22.14[20.81,23.37] & \textbf{1.05[0.94,1.16]} & 1.99[1.79,2.23] & 1.21[1.09,1.33] & 1.18[1.06,1.29] & 1.10[1.00,1.20] \\
gpt-4.1-mini vs gpt-5 & 23.37[22.22,24.39] & \textbf{1.10[1.01,1.21]} & 2.00[1.80,2.21] & 1.20[1.11,1.32] & 1.19[1.09,1.29] & 1.13[1.03,1.23] \\
gpt-4.1 vs gpt-4.1-mini & 2.47[1.66,3.39] & 1.19[1.09,1.31] & 1.83[1.63,2.01] & 1.42[1.30,1.56] & 1.31[1.18,1.45] & \textbf{1.19[1.06,1.32]} \\
gpt-4.1-mini vs gpt-5-mini & 23.20[21.98,24.29] & 1.22[1.12,1.33] & 2.25[2.02,2.49] & 1.36[1.25,1.48] & 1.33[1.22,1.44] & \textbf{1.22[1.12,1.33]} \\
gpt-4.1-mini vs gpt-4.1-mini & 2.38[1.59,3.32] & \textbf{1.40[1.27,1.52]} & 2.42[2.21,2.62] & 1.61[1.46,1.75] & 1.53[1.39,1.68] & 1.41[1.27,1.56] \\
gpt-5 vs gpt-5-mini & 26.15[25.53,26.65] & 2.05[1.91,2.21] & 2.44[2.30,2.60] & 2.11[1.98,2.26] & 1.95[1.81,2.10] & \textbf{1.88[1.75,2.03]} \\
gpt-5-mini vs gpt-5-mini & 26.47[26.00,26.83] & 2.11[1.98,2.27] & 2.78[2.61,2.94] & 2.17[2.04,2.31] & 2.03[1.90,2.16] & \textbf{1.93[1.81,2.07]} \\
gpt-5 vs gpt-5 & 26.76[26.66,26.87] & 2.14[2.02,2.25] & 2.37[2.24,2.51] & 2.21[2.11,2.32] & 2.03[1.92,2.13] & \textbf{1.96[1.87,2.07]} \\
\end{longtable}}


==> tables/ci/sm_n3_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{sm\_n3}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_sm_n3}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4o vs gpt-4o-mini & 1.70[1.47,1.95] & 15.36[13.86,16.88] & 1.33[1.09,1.59] & 0.20[0.13,0.27] & 0.19[0.13,0.25] & \textbf{0.19[0.13,0.25]} \\
gpt-4o vs gpt-4o & 2.00[1.75,2.25] & 13.72[12.29,15.20] & 1.40[1.14,1.65] & 0.28[0.21,0.37] & 0.28[0.21,0.37] & \textbf{0.26[0.19,0.35]} \\
gpt-4.1-mini vs gpt-4o-mini & 1.48[1.25,1.70] & 16.38[14.87,18.00] & 1.21[0.99,1.46] & 0.29[0.24,0.35] & 0.28[0.23,0.34] & \textbf{0.27[0.22,0.33]} \\
gpt-4.1 vs gpt-4o-mini & 1.63[1.41,1.87] & 17.68[16.25,19.09] & 1.63[1.36,1.90] & 0.32[0.26,0.38] & 0.31[0.25,0.38] & \textbf{0.31[0.25,0.37]} \\
gpt-4.1 vs gpt-4o & 1.88[1.69,2.10] & 13.25[11.67,14.84] & 1.07[0.92,1.24] & 0.32[0.24,0.41] & \textbf{0.31[0.23,0.39]} & 0.31[0.23,0.39] \\
gpt-4.1-mini vs gpt-4o & 1.88[1.65,2.10] & 13.12[11.62,14.61] & 1.05[0.88,1.22] & 0.31[0.24,0.40] & 0.31[0.24,0.40] & \textbf{0.31[0.24,0.40]} \\
gpt-4.1 vs gpt-4.1-mini & 2.21[1.93,2.47] & 11.93[10.31,13.50] & 1.21[0.98,1.47] & 0.62[0.51,0.72] & 0.62[0.51,0.72] & \textbf{0.51[0.42,0.61]} \\
gpt-4o-mini vs gpt-4o-mini & 1.67[1.40,1.95] & 14.10[12.61,15.64] & 0.94[0.76,1.15] & 0.54[0.46,0.63] & 0.53[0.45,0.62] & \textbf{0.52[0.44,0.61]} \\
gpt-4o-mini vs gpt-5 & 2.66[2.49,2.85] & 8.36[7.03,9.61] & 1.27[1.07,1.47] & 0.61[0.56,0.67] & 0.59[0.54,0.65] & \textbf{0.53[0.49,0.59]} \\
gpt-4.1-mini vs gpt-4.1-mini & 2.30[2.02,2.59] & 10.59[9.06,12.14] & 1.05[0.86,1.27] & 0.61[0.51,0.72] & 0.61[0.51,0.72] & \textbf{0.53[0.45,0.64]} \\
gpt-4o-mini vs gpt-5-mini & 2.78[2.60,2.96] & 8.65[7.23,10.06] & 1.40[1.19,1.61] & 0.65[0.61,0.71] & 0.65[0.61,0.71] & \textbf{0.57[0.53,0.64]} \\
gpt-4.1 vs gpt-5-mini & 2.88[2.68,3.09] & 9.21[7.56,10.79] & 1.37[1.16,1.60] & 0.69[0.61,0.76] & 0.68[0.60,0.76] & \textbf{0.61[0.53,0.69]} \\
gpt-4.1 vs gpt-4.1 & 2.36[2.10,2.67] & 10.75[9.13,12.27] & 1.21[0.96,1.45] & 0.86[0.79,0.95] & 0.86[0.79,0.95] & \textbf{0.64[0.56,0.74]} \\
gpt-4o vs gpt-5-mini & 3.00[2.78,3.24] & 8.86[7.30,10.36] & 1.38[1.18,1.59] & 0.73[0.64,0.83] & 0.72[0.63,0.82] & \textbf{0.65[0.56,0.75]} \\
gpt-4.1-mini vs gpt-5-mini & 3.06[2.87,3.26] & 9.56[7.94,11.25] & 1.52[1.31,1.75] & 0.76[0.69,0.84] & 0.75[0.68,0.82] & \textbf{0.66[0.59,0.73]} \\
gpt-4.1 vs gpt-5 & 3.06[2.85,3.28] & 8.06[6.53,9.55] & 1.41[1.21,1.62] & 0.74[0.67,0.82] & 0.73[0.66,0.82] & \textbf{0.66[0.59,0.74]} \\
gpt-4.1-mini vs gpt-5 & 3.17[2.94,3.39] & 8.12[6.62,9.65] & 1.36[1.16,1.57] & 0.78[0.68,0.87] & 0.75[0.66,0.84] & \textbf{0.68[0.58,0.77]} \\
gpt-4o vs gpt-5 & 3.08[2.87,3.29] & 6.51[5.27,7.82] & 1.22[1.06,1.40] & 0.75[0.67,0.83] & 0.75[0.67,0.83] & \textbf{0.70[0.62,0.77]} \\
gpt-5 vs gpt-5-mini & 5.05[4.91,5.16] & \textbf{0.03[0.01,0.09]} & 1.49[1.40,1.55] & 1.49[1.40,1.55] & 1.49[1.40,1.55] & 1.44[1.36,1.50] \\
gpt-5-mini vs gpt-5-mini & 5.08[4.94,5.20] & \textbf{0.02[0.00,0.07]} & 1.50[1.42,1.58] & 1.50[1.42,1.58] & 1.50[1.42,1.58] & 1.46[1.37,1.53] \\
gpt-5 vs gpt-5 & 5.12[5.01,5.20] & \textbf{0.01[0.00,0.04]} & 1.53[1.45,1.58] & 1.53[1.45,1.58] & 1.53[1.45,1.58] & 1.48[1.41,1.53] \\
\end{longtable}}


==> tables/ci/sm_n5_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{sm\_n5}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_sm_n5}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4.1 vs gpt-4o & 9.93[8.48,11.52] & 0.24[0.17,0.33] & 2.04[1.71,2.40] & 0.23[0.16,0.31] & 0.23[0.16,0.31] & \textbf{0.20[0.14,0.28]} \\
gpt-4.1-mini vs gpt-4o & 6.35[5.09,7.69] & 0.38[0.29,0.48] & 2.47[2.13,2.81] & 0.38[0.29,0.48] & 0.37[0.28,0.47] & \textbf{0.30[0.22,0.39]} \\
gpt-4.1 vs gpt-4o-mini & 6.47[5.12,7.86] & 0.39[0.30,0.51] & 2.96[2.59,3.35] & 0.38[0.28,0.49] & 0.36[0.27,0.47] & \textbf{0.34[0.25,0.44]} \\
gpt-4o vs gpt-4o & 7.51[6.06,9.00] & 0.50[0.40,0.61] & 1.66[1.36,1.96] & 0.48[0.38,0.58] & 0.44[0.35,0.54] & \textbf{0.36[0.27,0.46]} \\
gpt-4.1 vs gpt-4.1-mini & 5.63[4.48,6.77] & 0.49[0.39,0.61] & 2.44[2.14,2.76] & 0.49[0.39,0.61] & 0.48[0.38,0.59] & \textbf{0.39[0.30,0.48]} \\
gpt-4o vs gpt-4o-mini & 5.58[4.40,6.79] & 0.53[0.42,0.67] & 2.30[1.99,2.64] & 0.52[0.41,0.65] & 0.51[0.40,0.64] & \textbf{0.47[0.36,0.59]} \\
gpt-4.1 vs gpt-4.1 & 5.56[4.42,6.89] & 0.66[0.54,0.79] & 1.77[1.51,2.06] & 0.62[0.51,0.75] & 0.60[0.49,0.71] & \textbf{0.53[0.42,0.64]} \\
gpt-4.1-mini vs gpt-4o-mini & 5.19[4.15,6.37] & 0.63[0.51,0.77] & 2.90[2.57,3.27] & 0.63[0.51,0.77] & 0.63[0.51,0.77] & \textbf{0.55[0.44,0.68]} \\
gpt-4.1 vs gpt-5-mini & 6.75[5.37,8.09] & 0.78[0.67,0.89] & 2.43[2.07,2.79] & 0.76[0.66,0.88] & 0.76[0.66,0.87] & \textbf{0.71[0.59,0.83]} \\
gpt-4.1-mini vs gpt-4.1-mini & 5.90[4.67,7.00] & 0.85[0.71,0.98] & 3.34[3.04,3.64] & 0.85[0.71,0.98] & 0.84[0.70,0.97] & \textbf{0.72[0.60,0.83]} \\
gpt-4o vs gpt-5-mini & 5.21[3.96,6.56] & 0.82[0.73,0.93] & 2.25[1.95,2.60] & 0.82[0.72,0.93] & 0.81[0.71,0.92] & \textbf{0.78[0.67,0.88]} \\
gpt-4o-mini vs gpt-4o-mini & 5.67[4.61,6.84] & 0.90[0.76,1.07] & 2.76[2.46,3.08] & 0.89[0.76,1.04] & 0.87[0.73,1.00] & \textbf{0.81[0.67,0.95]} \\
gpt-4.1-mini vs gpt-5-mini & 3.55[2.67,4.59] & 0.97[0.86,1.07] & 3.08[2.72,3.48] & 0.97[0.86,1.07] & 0.94[0.83,1.04] & \textbf{0.89[0.78,1.00]} \\
gpt-4o-mini vs gpt-5-mini & 4.83[3.77,5.91] & 1.02[0.90,1.14] & 3.59[3.18,4.01] & 0.97[0.86,1.09] & 0.95[0.84,1.07] & \textbf{0.91[0.80,1.02]} \\
gpt-4.1 vs gpt-5 & 5.04[3.71,6.25] & 1.12[1.04,1.22] & 2.52[2.22,2.85] & 1.09[1.01,1.17] & 1.08[1.00,1.17] & \textbf{1.03[0.95,1.11]} \\
gpt-4o vs gpt-5 & 4.94[3.78,6.28] & 1.08[0.99,1.18] & 2.52[2.19,2.88] & 1.07[0.98,1.17] & 1.06[0.97,1.16] & \textbf{1.03[0.94,1.13]} \\
gpt-4.1-mini vs gpt-5 & 3.67[2.84,4.60] & 1.39[1.29,1.49] & 3.87[3.44,4.27] & 1.38[1.28,1.48] & 1.33[1.24,1.42] & \textbf{1.30[1.21,1.40]} \\
gpt-4o-mini vs gpt-5 & 3.68[2.90,4.53] & 1.44[1.31,1.57] & 4.25[3.82,4.67] & 1.39[1.27,1.51] & 1.38[1.26,1.49] & \textbf{1.33[1.22,1.44]} \\
gpt-5-mini vs gpt-5-mini & 4.47[3.56,5.51] & 2.27[2.13,2.43] & 2.50[2.33,2.67] & 2.10[1.97,2.23] & 2.06[1.93,2.20] & \textbf{1.84[1.69,1.99]} \\
gpt-5 vs gpt-5-mini & 3.14[2.58,3.84] & 2.52[2.36,2.67] & 2.70[2.55,2.86] & 2.30[2.16,2.43] & 2.29[2.15,2.43] & \textbf{2.12[1.98,2.25]} \\
gpt-5 vs gpt-5 & 2.82[2.66,3.08] & 3.00[2.88,3.11] & 3.19[3.09,3.31] & 2.73[2.62,2.83] & 2.73[2.61,2.83] & \textbf{2.54[2.43,2.64]} \\
\end{longtable}}


==> tables/ci/sm_n7_ci.tex <==
{\scriptsize\setlength{\tabcolsep}{2.5pt}\renewcommand{\arraystretch}{1.05}
\begin{longtable}{lrrrrrr}
\caption{Per-pair mean KL with 95\,\% bootstrap CI for game \texttt{sm\_n7}. Each cell is ``mean\,[lo,\,hi]'' in nats. Pairs sorted ascending by CQRE-pa mean. Boldface marks the lowest-mean equilibrium notion in each row.}\label{tab:appendix_ci_sm_n7}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{(continued)}}\\
\toprule
Model pair & Nash & Logit-QRE & Exact CQRE & CQRE sc. & CQRE pp. & CQRE-pa \\
\midrule
\endhead
\bottomrule
\endfoot
gpt-4.1 vs gpt-4o & 7.59[6.17,9.02] & 0.53[0.43,0.65] & 1.28[1.07,1.51] & 0.53[0.43,0.65] & 0.53[0.43,0.65] & \textbf{0.48[0.38,0.58]} \\
gpt-4o vs gpt-4o & 6.49[5.32,7.85] & 0.56[0.44,0.68] & 1.34[1.13,1.55] & 0.56[0.44,0.68] & 0.55[0.44,0.68] & \textbf{0.52[0.41,0.65]} \\
gpt-4.1 vs gpt-4.1 & 8.65[7.24,10.15] & 0.67[0.56,0.78] & 1.25[1.06,1.47] & 0.67[0.56,0.78] & 0.64[0.54,0.75] & \textbf{0.55[0.45,0.65]} \\
gpt-4.1-mini vs gpt-4o & 5.17[4.08,6.32] & 0.64[0.53,0.77] & 1.62[1.40,1.84] & 0.64[0.53,0.77] & 0.64[0.53,0.77] & \textbf{0.59[0.49,0.71]} \\
gpt-4o vs gpt-4o-mini & 7.19[5.94,8.55] & 0.64[0.51,0.78] & 1.68[1.46,1.91] & 0.64[0.51,0.78] & 0.64[0.51,0.78] & \textbf{0.59[0.48,0.71]} \\
gpt-4.1 vs gpt-4o-mini & 7.13[5.79,8.47] & 0.69[0.58,0.82] & 1.61[1.41,1.84] & 0.69[0.58,0.82] & 0.69[0.58,0.82] & \textbf{0.63[0.53,0.74]} \\
gpt-4.1 vs gpt-4.1-mini & 6.66[5.25,8.02] & 0.80[0.68,0.94] & 1.46[1.25,1.67] & 0.80[0.68,0.94] & 0.79[0.66,0.92] & \textbf{0.68[0.57,0.80]} \\
gpt-4.1-mini vs gpt-4o-mini & 6.74[5.53,8.13] & 0.91[0.78,1.05] & 1.95[1.75,2.15] & 0.91[0.78,1.05] & 0.90[0.78,1.05] & \textbf{0.85[0.73,0.97]} \\
gpt-4.1-mini vs gpt-4.1-mini & 4.08[3.24,5.07] & 1.23[1.10,1.35] & 2.05[1.83,2.28] & 1.23[1.10,1.35] & 1.20[1.09,1.33] & \textbf{1.06[0.95,1.19]} \\
gpt-4o-mini vs gpt-4o-mini & 6.29[5.14,7.47] & 1.28[1.09,1.47] & 1.88[1.68,2.09] & 1.28[1.09,1.47] & 1.27[1.08,1.46] & \textbf{1.14[0.96,1.31]} \\
gpt-4o vs gpt-5-mini & 22.84[21.85,23.77] & 1.24[1.12,1.36] & 1.99[1.80,2.19] & 1.21[1.10,1.32] & 1.20[1.09,1.32] & \textbf{1.17[1.06,1.29]} \\
gpt-4.1 vs gpt-5-mini & 22.61[21.50,23.69] & 1.36[1.24,1.49] & 1.97[1.79,2.15] & 1.30[1.19,1.43] & 1.30[1.19,1.43] & \textbf{1.25[1.14,1.36]} \\
gpt-4.1-mini vs gpt-5-mini & 22.77[21.61,23.82] & 1.51[1.37,1.65] & 2.38[2.18,2.59] & 1.46[1.33,1.60] & 1.45[1.32,1.59] & \textbf{1.39[1.26,1.53]} \\
gpt-4o-mini vs gpt-5-mini & 22.90[21.80,23.88] & 1.51[1.37,1.64] & 2.47[2.23,2.69] & 1.48[1.34,1.61] & 1.47[1.33,1.61] & \textbf{1.41[1.27,1.54]} \\
gpt-4o vs gpt-5 & 25.31[25.23,25.42] & 1.58[1.49,1.68] & 2.23[2.07,2.40] & 1.51[1.42,1.60] & 1.51[1.42,1.60] & \textbf{1.48[1.39,1.57]} \\
gpt-4.1 vs gpt-5 & 25.44[25.35,25.55] & 1.70[1.61,1.81] & 2.26[2.11,2.42] & 1.64[1.54,1.73] & 1.63[1.55,1.73] & \textbf{1.57[1.49,1.67]} \\
gpt-4o-mini vs gpt-5 & 25.46[25.38,25.56] & 1.72[1.64,1.82] & 2.70[2.52,2.89] & 1.68[1.60,1.78] & 1.68[1.60,1.78] & \textbf{1.63[1.55,1.72]} \\
gpt-4.1-mini vs gpt-5 & 25.51[25.20,25.73] & 1.88[1.76,2.01] & 2.90[2.72,3.10] & 1.84[1.72,1.96] & 1.84[1.72,1.96] & \textbf{1.77[1.65,1.90]} \\
gpt-5-mini vs gpt-5-mini & 26.65[26.27,26.94] & 3.03[2.85,3.22] & 2.59[2.47,2.71] & 2.59[2.47,2.71] & 2.59[2.47,2.71] & \textbf{2.45[2.33,2.58]} \\
gpt-5 vs gpt-5-mini & 27.00[26.82,27.17] & 3.26[3.08,3.43] & 2.74[2.64,2.85] & 2.74[2.64,2.85] & 2.74[2.64,2.85] & \textbf{2.64[2.53,2.76]} \\
gpt-5 vs gpt-5 & 27.57[27.50,27.63] & 3.83[3.76,3.89] & 3.11[3.05,3.15] & 3.11[3.05,3.15] & 3.11[3.05,3.15] & \textbf{3.04[2.98,3.08]} \\
\end{longtable}}

